Two-terminal Erasure Source-Broadcast with Feedback

We study the effects of introducing a feedback channel in the two-receiver erasure source-broadcast problem in which a binary equiprobable source is to be sent over an erasure broadcast channel to two receivers subject to erasure distortion constraints. The receivers each require a certain fraction of a source sequence, and we are interested in the minimum latency, or transmission time, required to serve them all. We first show that for a two-user broadcast channel, a point-to-point outer bound can always be achieved. We further show that the point-to-point outer bound can also be achieved if only one of the users, the stronger user, has a feedback channel. Our coding scheme relies on a hybrid approach that combines transmitting both random linear combinations of source symbols as well as a retransmission strategy.

==> SysModel/SysModel2_bak.tex <==
\section{{System Model}}
%\subsection{{}System Model}
%\section{Problem Formulation}
\label{sec:system_model_feedback}

%We first define the problem in Section~\ref{subsec:problem_definition}.  In Section~\ref{subsec:metrics}, we then discuss metrics that are of interest in the evaluation of broadcast codes and show how a solution to the problem in Section~\ref{subsec:problem_definition} can be used to address these metrics.

%\input{2_problem_formulation/problem_definition}
%\input{2_problem_formulation/metrics}

%%%\begin{figure*}
%%\begin{figure}
%%	\centering
%%%	\input{3/out/fig/schematic}
%%%	\includegraphics[scale=0.6]{3/out/fig/schematica}
%%%	\includegraphics[scale=0.75]{out/fig/schematic}
%%%	\includegraphics[scale=0.8]{2_problem_formulation/fig/schematicE}
%%	\includegraphics{2_problem_formulation/fig/schematicE}
%%%	\includegraphics[width=0.6\textwidth]{outer_bound.png}
%%	\caption{Broadcasting an equiprobable binary source over an erasure broadcast channel.}
%%	\label{fig:schematic}
%%%\end{figure*}
%%\end{figure}

%We begin by presenting our joint source-channel coding formulation which is illustrated in Fig.~\ref{fig:schematic}.

%\begin{figure*}
%%%%%\begin{figure}
%%%%%	\centering
%%%%%%	\input{fig/schematicE}
%%%%%%	\includegraphics[scale=0.95]{fig/schematic}
%%%%%	\includegraphics[scale=0.75]{fig/schematic}
%%%%%%	\includegraphics[scale=0.75]{SysModel/fig/schematic_arrow}
%%%%%	\caption{Broadcasting an equiprobable binary source over an erasure broadcast channel.}
%%%%%	\label{fig:schematic}
%%%%%%\end{figure*}
%%%%%\end{figure}

%The problem is illustrated in Fig.~\ref{fig:schematic}.  
We first consider a version of the erasure-source broadcast problem involving universal feedback, after which, we consider the case of one-sided feedback in Section~\ref{}. Our problem involves communicating a binary memoryless source $\{S(t)\}_{t=1,2, \ldots}$ to two users over an erasure broadcast channel with feedback.  %Let $\mathcal{S}^{N}$ be the set of all $N$-vectors with components in $\mathcal{S}$, and denote $(S(1), S(2), \ldots , S(N))$ as $S^{N}$.  For convenience, we will also denote the set $\{1,2,\dots,N\}$ as $[N]$.
%
%\begin{figure}
%	\centering
%%	\input{3/fig/schematic}
%	\includegraphics[scale=0.8]{fig/schematicE}
%%%	\includegraphics[width=0.6\textwidth]{outer_bound.png}
%	\caption{Broadcasting an equiprobable binary source over an erasure broadcast channel with individual bandwidth mismatches.}
%	\label{fig:schematicE}
%\end{figure}
%
The source produces equiprobable symbols in $\mathcal{S}=\{0,1\}$ and is communicated by an encoding function that produces the channel input sequence $X^{W} = (X(1),  \dots , X(W))$, where $X(t)$ denotes the $t^{\mathrm{th}}$ channel input taken from the alphabet $\mathcal{X} = \{0, 1\}$.  We assume that 
$X(t)$ is a function of the source as well as the channel outputs of all users prior to time $t$.  
%The encoding function produces the channel input sequence $X^{W} = (X(1),  \dots , X(W))$, where $X(t)$ denotes the $t^{\mathrm{th}}$ channel input taken from the alphabet $\mathcal{X} = \{0, 1\}$.  %Note here that our notation defines $X^{n}$ as the first $n$ channel symbols sent. %which is also taken from the alphabet $\mathcal{S}$.  %

% Original
%Let $Y_{i}(t)$ be the channel output observed by user $i$ on the $t^{\mathrm{th}}$ channel use for $i \in [n]$ and $t \in [W]$.  Our channel model is an erasure channel.  In particular, let $\epsilon_i$ denote the erasure rate of the channel corresponding to user~$i$.  Without loss of generality, we will assume that $0 < \epsilon_{1} < \epsilon_{2} < \ldots < \epsilon_{n} < 1$.  Then $Y_{i}(t)$ exactly reproduces the channel input $X(t)$ with probability $(1 - \epsilon_i)$ and otherwise indicates an erasure event, which happens with probability $\epsilon_i$.  We let $Y_{i}(t)$ take on values in the alphabet $\mathcal{Y} = \{0, 1, \star\}$ so that an erasure event is represented by `$\star$,' the erasure symbol.  We associate user~$i$ with the state sequence $(N_i(t))_{t \in [W]}$, which is defined such that $N_{i}(t) = 1$ if $Y_i(t)$ was erased and $N_i(t) = 0$ otherwise.  The channel we consider is memoryless in the sense that $N_{i}(t)$ is drawn i.i.d.\ from a $\operatorname{Bern}(1 - \epsilon_{i})$ distribution.

Let $Y_{i}(t)$ be the channel output observed by user $i$ on the $t^{\mathrm{th}}$ channel use for $i \in [n] \triangleq \{1, 2, \ldots, n\}$. %$\mathcal{U}= \{1, 2, 3\}$ and $t \in [W] = \{1, \ldots, W\}$.  %Our channel model is a binary erasure broadcast channel. % as shown in Fig.~\ref{fig:schematic}.  
%In particular, let $\epsilon_i$ denote the erasure rate of the channel corresponding to user~$i$, where we assume that $0 < \epsilon_{1} < \epsilon_{2} < \ldots < \epsilon_{n} < 1$.  This is without loss of generality since we can address {{}all} users that experience identical erasure rates by serving the {{}one} with the most stringent distortion requirement.  
%In particular, if $\epsilon_i$ denotes the erasure rate of the channel corresponding to user~$i$, our model specifies that $Y_{i}(t)$ exactly reproduces the channel input $X(t)$ with probability $(1 - \epsilon_i)$ and otherwise indicates an erasure event, which happens with probability $\epsilon_i$.  
We let $Y_{i}(t)$ take on values in the alphabet $\mathcal{Y} = \{0, 1, \star\}$ so that an erasure event is represented by `$\star$'.   
%
We associate user~$i$ with the state sequence $\{Z_i(t)\}_{t \in [W]}$, which represents the noise on user~$i$'s channel, where $Z_i(t) \in \mathcal{Z} \triangleq \{0,1\}$,  and  $Y_i(t)$ will be erased if $Z_{i}(t) = 1$ and $Y_{i}(t) = X(t)$ if $Z_i(t) = 0$.  The channel we consider is memoryless in the sense that $Z_{i}(t)$ is drawn i.i.d.\ from a $\operatorname{Bern}(\epsilon_{i})$ distribution, where
$\epsilon_i$ denotes the erasure rate of the channel corresponding to user~$i$.
%\textcolor{blue}{We assume that the erasure rates are known to both the transmitter and receiver. If such channel knowledge is not possible, we can take the standard approach of interpreting a broadcast channel as an abstraction for a \emph{compound channel}~\cite{CT}.  In such a situation, the compound channel is a channel that randomly takes on one of many potential states for the duration of transmission.  We model this by considering a broadcast channel whose constituent channels correspond to these potential channel states.}
%{}{Note that in our setup, the erasure rates for each user are assumed to be known. However, our setup also models the 
%compound channel~\cite{CT}, where an erasure rate is not known and instead belong to a collection of possible states, with each 
%state corresponding to one virtual user in our system.}

%Let $Y_{i}(t)$ be the channel output observed by user $i$ on the $t^{\mathrm{th}}$ channel use for $i \in [n]$ and $t \in [W]$.  Our channel model is an erasure channel.  In particular, $Y_{i}(t)$ either exactly reproduces the channel input $X(t)$ or otherwise indicates an erasure event.  We let $Y_{i}(t)$ take on values in the alphabet $\mathcal{Y} = \{0, 1, \star\}$ so that an erasure event is represented by `$\star$,' the erasure symbol.  Let $\epsilon_i$ denote the erasure rate of the channel corresponding to user~$i$.  Without loss of generality, we assume that $0 < \epsilon_{1} < \epsilon_{2} < \ldots < \epsilon_{n} < 1$.  We associate user~$i$ with the state sequence $(N_i(t))_{t \in [W]}$, where $N_i(t) \in \{0,1\}$.  The state sequence represents the noise on user~$i$'s channel and we will have that $Y_i(t)$ is erased if $N_{i}(t) = 1$ and $Y_{i}(t) = X(t)$ if $N_i(t) = 0$.  The channel we consider is memoryless in the sense that $N_{i}(t)$ is drawn i.i.d.\ from a $\operatorname{Bern}(1 - \epsilon_{i})$ distribution.

%\begin{equation}
%%\label{eq:channel_model}
%	Y_{i}(t) = X(t) \cdot N_{i}(t),
%\end{equation}
%
%where $N_{i}(l)$ is a $\operatorname{Bern}(1 - \epsilon_{i})$ random variable representing the noise at user $i$'s $l^{\mathrm{th}}$ channel output.  The channel is memoryless in the sense that $N_{i}(l)$ is drawn i.i.d.\ from a $\operatorname{Bern}(1 - \epsilon_{i})$ distribution.  %Specifically, the statistics of $N_{i}(l)$ are such that
%
%\begin{equation}
%\label{eq:nstat}
%	N_{i}(l) =
%	\begin{cases}
%		0 & \text{with probability} \ \epsilon_{i}, \\
%		1 & \text{with probability} \ 1 - \epsilon_{i}.
%	\end{cases}
%\end{equation}
%
%Thus, $Y_{i}(l)$ takes on values in the alphabet $\mathcal{Y} = \{-1, 0, +1\}$ and we interpret $Y_{i}(l)$ as the output of an erasure channel, with erasure probability $\epsilon_{i}$, when $X(l)$ is the channel input (see Section~\ref{sec:erased_rv} for a discussion of the erasure channel model).
%
%Thus, $Y_{i}(l)$ takes on values in the alphabet $\mathcal{Y} = \{-1, 0, +1\}$.  If we define `0' as the erasure symbol, we can interpret $Y_{i}(l)$ as the output of an erasure channel with erasure probability $\epsilon_{i}$ when $X(l)$ is the channel input. Without loss of generality, we will assume that $0 < \epsilon_{1} < \epsilon_{2} < \ldots < \epsilon_{n} < 1$. %Users on channels with the same erasure probability are represented by a user of the smallest distortion

%Now although the length-$n$ channel input is broadcasted to both users, we will assume that due to each user's delay constraint, the $i^{\mathrm{th}}$ user reconstructs the source after observing only the first $n_{i}$ channel input symbols, denoted as $X^{n_{i}}$, where $n_{i} \leq n$.  Specifically, we have that $n = \max(n_{1}, n_{2})$.

The problem we consider involves causal feedback  that is universally available.  That is, at time $T$, we assume that $\{Z_1(t), Z_2(t), \ldots,  Z_n(t)\}_{t=1, 2, \ldots, T-1}$ is available to the transmitter and all receivers. 
After $W$ channel uses, user $i$ utilizes the feedback and his own channel output to reconstruct the source as a length-$N$ sequence, denoted as $\hat{S}_{i}^{N}$.  We will be interested in a fractional recovery requirement so that each symbol in $\hat{S}_{i}^{N}$ either faithfully recovers the corresponding symbol in $S^{N}$, or otherwise a failure is indicated with an erasure symbol, i.e., we do not allow for any bit flips.

More precisely, we choose the reconstruction alphabet $\mathcal{\hat{S}}$ to be an augmented version of the source alphabet so that $\mathcal{\hat{S}} = \{0, 1, \star\}$, where the additional `$\star$' symbol indicates an erasure symbol.  Let $\mathcal{D} = [0,1]$ and $d_i \in \mathcal{D}$ be the distortion user $i$ requires.  We then express the constraint that an achievable code ensures that each user $i \in [n]$ achieves a fractional recovery of $1 - d_{i}$ with the following definition.

%by first defining the set $D_{i}(\hat{S}_{i}^{N}) = \{l \in [N] : \hat{S}_{i}(l) = 0\}$.

%Note that the we have taken the reconstruction alphabet to be an augmented version of the source alphabet by adding the additional `0' symbol, which we interpret as an erasure symbol.  In our reconstruction, we require that $\hat{S}_{i}^{N}$ is such that for $l \in [N]$, $\hat{S}_{i}(l) = S(l)$ or $\hat{S}_{i}(l) = 0$.  In other words, we do not allow any bit flips in our reconstruction so that $\hat{S}_{i}(l)$ either faithfully reproduces $S(l)$ or otherwise outputs an erasure symbol.


%%%On a symbol-by-symbol basis, we measure the reconstruction's fidelity with the erasure distortion $d_{E}: \mathcal{S} \times \hat{\mathcal{S}} \to \{0,1, \infty\}$ given by
%%%%Depending on the distortion measure we use, $\mathcal{\hat{S}}$ can either be a binary source alphabet or the extended alphabet $\mathcal{\hat{S}_{E}} = \{-1, 0, 1\}$, where `0' denotes the source erasure symbol.
%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%On the other hand, when the output alphabet can include the source erasure symbol as in the second case, then on a symbol-by-symbol comparison, the reconstruction's fidelity is measured with the erasure distortion $d_{E} : \mathcal{S} \times \mathcal{\hat{S}_{E}} \to \{0, 1, \infty\}$, given by
%%%
%%%\begin{equation}
%%%\label{eq:symbol_distortion1}
%%%	d_{E}(s, \hat{s}) =
%%%	\begin{cases}
%%%		0 & \text{if } \hat{s} = s, \\
%%%		1 & \text{if } \hat{s} = 0 \\
%%%		\infty & \text{otherwise}.
%%%	\end{cases}
%%%\end{equation}
%%%%
%%%The per-letter distortion of a vector is then defined as $d(s^{k}, \hat{s}^{k}) = \frac{1}{k} \Sigma_{m=1}^{k} d(s_{m}, \hat{s}_{m})$.
%%%
%%%%\begin{equation}
%%%%\label{eq:vector_distortion1}
%%%%	d(s^{k}, \hat{s}^{k}) = \frac{1}{k} \sum\limits_{i=1}^k d(s_{i}, \hat{s}_{i}).
%%%%\end{equation}
%%%%
%%%%where $d(\cdot, \cdot)$ can be either $d_{H}(\cdot, \cdot)$ or $d_{E}(\cdot, \cdot)$.
%%%
%%%%We point out that with the erasure distortion measure,  a finite distortion value indicates that we are certain about the accuracy of the non-erased symbols in our reconstruction, while the actual value of the distortion is a measure of the proportion of bits that we are unsure about, i.e., that have been erased in the reconstruction.
%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
%%%
%%%We point out that with the erasure distortion measure,  a finite distortion value indicates that we are certain about the accuracy of the non-erased symbols in our reconstruction, while the actual value of the distortion is a measure of the proportion of bits that we are unsure about, i.e., that have been erased in the reconstruction.  We now define the components of our problem.

\begin{mydef}
\label{def:code_two_users_feedback}
	An $(N, W, d_{1}, d_{2}, \ldots, d_{n})$ code for source $S$ on the erasure broadcast channel with feedback consists of	
	\begin{enumerate}
		\item a sequence of encoding functions $f_{i, N} : \mathcal{S}^{N} \times  \prod_{j = 1}^{n} \mathcal{Z}^{i-1} \to \mathcal{X}$ for $i \in [W]$, such that $X(i) = f_{i, N}(S^{N}, Z_1^{i -1}, Z_2^{i -1}, \ldots, Z_n^{i - 1})$, and
		
		\item $n$ decoding functions $g_{i,N} : \mathcal{Y}^{W} \times  \mathcal{Z}^{nW} \to \mathcal{\hat{S}}^{N}$ s.t.\ $\hat{S}_{i}^{N} = g_{i,N}(Y_{i}^{W}, Z_1^{W}, Z_2^{W}, \ldots, Z_n^{W})$, $i \in [n]$,
		\begin{enumerate}
			\item $\hat{S}_{i}^{N}$ is such that for $t \in [N]$, if $\hat{S}_{i}(t) \neq S(t)$, then $\hat{S}_{i}(t) = \star$,
%			\item $\mathbb{E}   \left\vert{D_{i}(\hat{S}_{i}^{N})}\right\vert \leq d_{i}$
			\item $\mathbb{E}   \left\vert{\{t \in [N] \mid \hat{S}_{i}(t) = \star\}}\right\vert \leq N d_{i}$,
		\end{enumerate}
		 	
%	$\mathbb{E}d(S^{k}, g_{i}( X^{n} \cdot N_{i}^{n})) \leq D_{i}$ holds for $i \in \{1,2\}$		
	\end{enumerate}
	
%	where $\mathbb{E}(\cdot)$ is the expectation operation and $\vert A \vert$ denotes the cardinality of set $A$.
\end{mydef}

%\begin{mydef}
%\label{def:code}
%	An $(N, W, d_{1}, d_{2}, d_{3})$ code for source $S$ on the erasure broadcast channel consists of
%	\begin{enumerate}
%		\item a sequence of encoding functions $f_{i, N} : \mathcal{S}^{N} \times  \prod_{j = 1}^{3} \mathcal{N}^{i-1} \to \mathcal{X}$ for $i \in [W]$, such that $X(i) = f_{i, N}(S^{N}, N_1^{i -1}, N_2^{i -1}, N_3^{i - 1})$, and
%		
%		\item three decoding functions $g_{i,N} : \mathcal{Y}^{W} \times  \prod_{j = 1}^{3} \mathcal{N}^{W} \to \mathcal{\hat{S}}^{N}$ s.t.\ $\hat{S}_{i}^{N} = g_{i,N}(Y_{i}^{W}, N_1^{W}, N_2^{W}, N_3^{W})$, $i \in \{1, 2, 3\}$,
%		\begin{enumerate}
%			\item $\hat{S}_{i}^{N}$ is such that for $t \in [N]$, if $\hat{S}_{i}(t) \neq S(t)$, then $\hat{S}_{i}(t) = \star$,
%%			\item $\mathbb{E}   \left\vert{D_{i}(\hat{S}_{i}^{N})}\right\vert \leq d_{i}$
%			\item $\mathbb{E}   \left\vert{\{t \in [N] \mid \hat{S}_{i}(t) = \star\}}\right\vert \leq N d_{i}$,
%		\end{enumerate}
%		 	
%%	$\mathbb{E}d(S^{k}, g_{i}( X^{n} \cdot N_{i}^{n})) \leq D_{i}$ holds for $i \in \{1,2\}$		
%	\end{enumerate}
%	
%%	where $\mathbb{E}(\cdot)$ is the expectation operation and $\vert A \vert$ denotes the cardinality of set $A$.
%\end{mydef}

%A point is now made about the modelling of latencies in our problem.  We define the \emph{latency} or \emph{bandwidth expansion factor} $b \in [0, \infty )$, as the number of channel uses per source symbol that are delivered over the broadcast channel, i.e., $b \triangleq n/k$.  This is to say that $b \cdot k$ channel uses are required before both users can reconstruct $S^{k}$ subject to their distortion constraints.  Our problem is now defined as characterizing the achievable latency region under a given pair of distortion constraints as per the next definition.

%A point is now made about the modelling of delays in our problem.  We define the bandwidth expansion factor $b \in [0, \infty )$, as $b = n/k$.  We interpret $b$ as the normalized latency (in units of ``channel uses per source symbol''), before both users can reconstruct $S^{k}$ subject to their distortion constraints.  Our problem is now defined as characterizing the achievable distortion region under a given bandwidth expansion factor as per the next definition.
%
We mention that in our problem formulation, we assume that all receivers have causal knowledge of $(Z_{1}^{t-1}, Z_{2}^{t-1}, \ldots, Z_{n}^{t-1})$ at time $t$.  That is, each receiver has causal knowledge of which packets were received.  This can be made possible, for example, through the control plane of a network.

We define the {\it latency} that a given code requires before all users can recover their desired fraction of the source as follows:
\begin{mydef}
	The latency, $w$, of an~$(N, W, d_{1}, d_{2}, \ldots, d_{n})$ code is the number of channel uses per source symbol that the code requires to meet all distortion demands, i.e., $w = W/N$.
\end{mydef}
%
Our goal is to characterize the achievable latencies under a prescribed distortion vector,
as per the following definition:
\begin{mydef}
\label{def:achievable_general_feedback}
	Latency $w$ is said to be $(d_{1}, d_{2}, \ldots,  d_{n})$-achievable over the erasure broadcast channel if for every $\delta > 0$, there exists for sufficiently large $N$, an $(N, wN, \hat{d}_{1}, \hat{d}_{2}, \ldots, \hat{d}_{n})$ code such that for all $i \in [n]$, $d_{i}+\delta \geq \hat{d}_{i}$.
	
%	\begin{equation}
%		D_{i}+\delta \geq d_{i},  \quad i \in \{1, 2\}.
%	\end{equation}	
%	Alternatively, we may occasionally say that the tuple $(b, D_{1}, D_{2})$ is achievable if the latency $b$ is $(D_{1}, D_{2})$-achievable.
	
%The achievable latency region is the set of all achievable latencies under the prescribed distortion vector.

\end{mydef}

%In the remaining sections, we consider the cases $n=2$ and $n=3$.  We will also make a mention whenever the strategies we use for these cases can be generalized for $n$ users.  
In this chapter, we consider the case when $n=2$.  We study the case when $n=3$ in the following chapter.  We will also make a mention whenever the strategies we use for these cases can be generalized for $n$ users.  
%While this may seem to be an oversimplification, it is worth noting that to the authors' best knowledge, a solution is also not known for the related channel coding problem involving $n$ users~\cite{GGT}.

%\begin{remark}
%\label{rem:deps}
%Throughout this paper we will assume that for each user $i \in [n]$, we have that $d_i < \epsilon_i$. Any user with $d_i \ge \epsilon_i$ will be trivially satisfied by the systematic portion of our segmentation-based coding scheme.  Furthermore, we will show in Lemma~\ref{lem:bn1} that within our class of coding schemes, such a systematic portion can be transmitted without loss of optimality when at least one user satisfies $d_i < \epsilon_i$. Finally, if every user satisfies $d_i \ge \epsilon_i$, a simple uncoded transmission scheme is easily shown to be optimal.
%\end{remark}
%
%\begin{remark}
%	While our system model has assumed binary alphabets for both the source and channel input sequences, our results can be easily extended to larger alphabet sizes for the purpose of applying our results to packet erasure networks.
%\end{remark}


%For convenience, throughout this paper, for any positive integer $k$, we shorthand the set $\{1,2,\dots,k\}$ as $[k].$
%
%Consider broadcasting a length-$N$ binary sequence $S = \{s(j)\}_{j\in[N]}$ from a source to $n$ receivers over independent memoryless binary erasure channels. For $i\in[n]$, denote the erasure rate of the channel between the source and receiver $i$ as $\epsilon_i$. Applying some encoding scheme to $S$, the source generates and broadcasts the coded binary sequence $X=\{x_j\}_{j\ge1}$. Each receiver $i$ retrieves from the channel a sequence $Y^i = \{y_{j}^i\}_{j\ge1}$ where $y_{j}^i \in \{0,1,e\}$, $e$ indicating an erasure. Denote $Y^{i,W} = \{y_{j}^i\}_{j\in[W]}$ as the truncation of $Y^i$ up to the $W$th symbol. Receiver $i$ reconstructs from $Y^{i,W}$ a copy $\hat S^{i,W}=\{\hat s_{j}^{i,W}\}_{j\in[N]},$ where $\hat s_{j}^{i,W}\in\{0,1,e\}.$
%
%%\subsection{Erasure Distortion}
%We consider a symbol-by-symbol based erasure reconstruction distortion measure $D_e: \{0,1\}\times \{0,1,e\}\mapsto \mathds R$ defined as
%\begin{align*}
%D_E(s,\hat s) = \left\{\begin{array}{lr} 0,& \textnormal{if } \hat s=s\\ 1, & \textnormal{if } \hat s\ne s, \hat s\ne e\\ \infty,& \textnormal{if } \hat s=e \end{array}\right.
%\end{align*}
%%for symbols $s\in\{0,1\}$ and $\hat s\in\{0,1,e\}$,
%and
%\begin{align*}
%D(S,\hat S^{i,W}) =  \frac{1}{N}\sum_{j\in[N]} D_E(s_j,\hat s_{j}^{i,W}).
%\end{align*}
%for the source sequence $S$ and the sequence $\hat S^{i,W}$ reconstructed by user $i$ from the first $W$ symbols of the channel output sequence $Y^{i,W}$.
%
%Now our problem is to upper bound and lower bound the minimum $W$, or $w=W/N,$ which we refer to as the {\it latency}, that guarantees $\mathds E[ D(S,\hat S^{i,W})]\le d_i$ for all $i\in[n]$,
%where $d_i$ is the given distortion requirement of user $i$.
%
%Clearly, $w$ is trivially lower bounded by $\max_{i\in[n]}\{\frac{1-d_i}{1-\epsilon_i}\}$. In the next section, we provide an upper bound of $w$ and the achieving coding scheme. We show that the upper bound is achieved with a coding scheme that sends a part of the source sequence uncoded, partitions the rest of the source sequence into a number of segments, and encodes each segment by a systematic optimal erasure code. The optimal segmentation can be found by solving a linear programming problem. We also show in Sec.~\ref{sec:jscc} that the segmentation-based scheme is equivalent to the Mittal-Phamdo~\cite{} scheme for erasure channels.

%\input{SysModel/individual_code}




%\input{SysModel/JSCC_approach3}










==> fig/latex_src/char_header.tex <==
% ABBREVIATIONS FOR CHARACTERS IN VARIOUS FONTS

% STANDARD CHARACTERS

\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bah}{{\hat{\ba}}}
\newcommand{\ah}{{\hat{a}}}
\newcommand{\Ah}{{\hat{A}}}
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\at}{{\tilde{a}}}
\newcommand{\bat}{{\tilde{\ba}}}
\newcommand{\At}{{\tilde{A}}}
\newcommand{\bA}{{\mathbf{A}}}
\newcommand{\ac}{a^{\ast}}

\newcommand{\bb}{{\mathbf{b}}}
\newcommand{\bbt}{{\tilde{\bb}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\tb}{{\tilde{b}}}
\newcommand{\tB}{{\tilde{B}}}
\newcommand{\hb}{{\hat{b}}}
\newcommand{\hB}{{\hat{B}}}
\newcommand{\bB}{{\mathbf{B}}}

\newcommand{\bc}{{\mathbf{c}}}
\newcommand{\bch}{{\hat{\mathbf{c}}}}
\newcommand{\bC}{{\mathbf{C}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\ct}{{\tilde{c}}}
\newcommand{\Ct}{{\tilde{C}}}
\newcommand{\ctc}{\ct^{\ast}}

\newcommand{\bd}{{\mathbf{d}}}
\newcommand{\bD}{{\mathbf{D}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\hd}{{\hat{d}}}  % old: \dh
\newcommand{\dt}{{\tilde{d}}}
\newcommand{\bdt}{{\tilde{\bd}}}
\newcommand{\Dt}{{\tilde{D}}}
\newcommand{\dtc}{\dt^{\ast}}

\newcommand{\et}{{\tilde{e}}}
\newcommand{\bfe}{{\mathbf{e}}}
\newcommand{\bE}{{\mathbf{E}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cEt}{{\tilde{\cE}}}
\newcommand{\cEb}{{\bar{\cE}}}
\newcommand{\bcE}{{\mathbf{\cE}}}  % bf cal E doesn't exist

\newcommand{\bff}{{{\mathbf{f}}}}
\newcommand{\bF}{{\mathbf{F}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\ft}{{\tilde{f}}}
\newcommand{\Ft}{{\tilde{F}}}
\newcommand{\Fh}{{\hat{F}}}
\newcommand{\ftc}{\ft^{\ast}}
\newcommand{\bft}{{\tilde{\bff}}}
\newcommand{\bFt}{{\tilde{\bF}}}
\newcommand{\fh}{{\hat{f}}}

\newcommand{\bg}{{\mathbf{g}}}
\newcommand{\gt}{{\tilde{g}}}
\newcommand{\bgt}{{\tilde{\bg}}}
\newcommand{\bG}{{\mathbf{G}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\Gt}{{\tilde{\bG}}}
\newcommand{\Ge}{{G_\mathrm{eff}}}


\newcommand{\hti}{{\tilde{h}}}
\newcommand{\Hti}{{\tilde{H}}}
\newcommand{\bh}{{\mathbf{h}}}
\newcommand{\bht}{{\tilde{\bh}}}
\newcommand{\Hh}{{\hat{H}}}
\newcommand{\bH}{{\mathbf{H}}}
\newcommand{\bHh}{{\hat{\mathbf{H}}}}

\newcommand{\ih}{{\hat{\imath}}}
\newcommand{\bI}{{\mathbf{I}}}
\newcommand{\cI}{{\mathcal{I}}}

\newcommand{\jh}{{\hat{\jmath}}}
\newcommand{\bJ}{{\mathbf{J}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\Jt}{{\tilde{J}}}

\newcommand{\bk}{{\mathbf{k}}}
\newcommand{\bK}{{\mathbf{K}}}
\newcommand{\Kt}{{\tilde{K}}}
\newcommand{\Kh}{{\hat{K}}}
\newcommand{\cK}{{\mathcal{K}}}

\newcommand{\cl}{\ell}
\newcommand{\bL}{{\mathbf{L}}}
\newcommand{\cL}{{\mathcal{L}}}

\newcommand{\mb}{{\mathbf{m}}}
\newcommand{\mh}{{\hat{m}}}
\newcommand{\bM}{{\mathbf{M}}}
\newcommand{\bm}{{\mathbf{m}}}
\newcommand{\cM}{{\mathcal{M}}}


\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\CN}{{\mathcal{CN}}}
\newcommand{\Nt}{{\tilde{N}}}
\newcommand{\tN}{{\tilde{N}}}  % backward compatibility

\newcommand{\bo}{{\mathbf{o}}}
\newcommand{\cO}{{\mathcal{O}}}

\newcommand{\bp}{{\mathbf{p}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\ph}{{\hat{p}}}
\newcommand{\Ph}{{\hat{P}}}
\newcommand{\Pt}{{\tilde{P}}}
\newcommand{\Ptt}{{\tilde{\tilde{P}}}}
\newcommand{\bq}{{\mathbf{q}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\bQ}{{\mathbf{Q}}}

\newcommand{\br}{{\mathbf{r}}}
\newcommand{\bR}{{\mathbf{R}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\Rt}{{\tilde{R}}}

\newcommand{\sh}{{\hat{s}}}
\newcommand{\sck}{{\check{s}}}
\newcommand{\shh}{{\Hat{\Hat{s}}}}
\newcommand{\bs}{{\mathbf{s}}}
\newcommand{\bsh}{{\hat{\mathbf{s}}}}
\newcommand{\bsc}{{\check{\mathbf{s}}}}
\newcommand{\bshh}{{\Hat{\Hat{\mathbf{s}}}}}
\newcommand{\bS}{{\mathbf{S}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\st}{{\tilde{s}}}

\newcommand{\bT}{{\mathbf{T}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bU}{{\mathbf{U}}}
\newcommand{\bUt}{{\tilde{\bU}}}
\newcommand{\ut}{{\tilde{u}}}
\newcommand{\cU}{{\mathcal{U}}}

\newcommand{\vh}{{\hat{v}}}
\newcommand{\bv}{{\mathbf{v}}}
\newcommand{\bV}{{\mathbf{V}}}
\newcommand{\cV}{{\mathcal{V}}}

\newcommand{\bw}{{\mathbf{w}}}
\newcommand{\bW}{{\mathbf{W}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\wt}{{\tilde{w}}}

\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\bxt}{{\tilde{\bx}}}
\newcommand{\xt}{{\tilde{x}}}
\newcommand{\Xt}{{\tilde{X}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\bXt}{{\tilde{\bX}}}
\newcommand{\xh}{{\hat{x}}}
\newcommand{\xc}{{\check{x}}}
\newcommand{\xhh}{{\Hat{\Hat{x}}}}
\newcommand{\bxh}{{\hat{\bx}}}
\newcommand{\bxc}{{\check{\bx}}}
\newcommand{\bxhh}{{\Hat{\hat{\bx}}}}

\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\byt}{{\tilde{\by}}}
\newcommand{\bY}{{\mathbf{Y}}}
\newcommand{\Yt}{{\tilde{Y}}}
\newcommand{\yt}{{\tilde{y}}}
\newcommand{\yh}{{\hat{y}}}

\newcommand{\zt}{{\tilde{z}}}
\newcommand{\zh}{{\hat{z}}}
\newcommand{\bz}{{\mathbf{z}}}
\newcommand{\bZ}{{\mathbf{Z}}}
\newcommand{\cZ}{{\mathcal{Z}}}

% GREEK CHARACTERS

\newcommand{\al}{\alpha}
\newcommand{\bal}{{\boldsymbol{\al}}}
\newcommand{\balh}{{\hat{\boldsymbol{\al}}}}
\newcommand{\alh}{{\hat{\al}}}
\newcommand{\aln}{{\bar{\al}}}

\newcommand{\bt}{\boldsymbol{t}}
%\newcommand{\bt}{\beta}
\newcommand{\btt}{{\tilde{\bt}}}
\newcommand{\btht}{{\hat{\bt}}}

\newcommand{\g}{\gamma}
\newcommand{\G}{\Gamma}
\newcommand{\bGa}{{\boldsymbol{\Gamma}}}
\newcommand{\gh}{{\hat{\g}}}

\newcommand{\de}{\delta}
\newcommand{\del}{\delta}
\newcommand{\De}{\Delta}
\newcommand{\Deh}{{\hat{\Delta}}}
\newcommand{\bde}{{\boldsymbol{\de}}}
\newcommand{\bDe}{{\boldsymbol{\De}}}

\newcommand{\e}{\epsilon}
\newcommand{\eps}{\varepsilon}

\newcommand{\etah}{{\hat{\eta}}}
\newcommand{\bpi}{{\boldsymbol{\pi}}}

\newcommand{\pht}{{\tilde{\phi}}}
\newcommand{\Pht}{{\tilde{\Phi}}}

\newcommand{\pst}{{\tilde{\psi}}}
\newcommand{\Pst}{{\tilde{\Psi}}}

\newcommand{\s}{\sigma}
\newcommand{\sih}{\hat{\sigma}}

\newcommand{\z}{\zeta}
\newcommand{\ztt}{{\tilde{\z}}}
\newcommand{\ztb}{{\bar{\z}}}

% \newcommand{\th}{\theta} % symbol name used by other latex package
\newcommand{\thh}{{\hat{\theta}}}
\newcommand{\Thh}{{\hat{\Theta}}}
\newcommand{\Th}{\Theta}
\newcommand{\bth}{{\boldsymbol{\theta}}}
\newcommand{\bTh}{{\boldsymbol{\Theta}}}
\newcommand{\bThh}{{\hat{\bTh}}}
\newcommand{\Tht}{{\tilde{\Theta}}}

\newcommand{\la}{\lambda}
\newcommand{\La}{\Lambda}
\newcommand{\lam}{\lambda}  % backward compatibility
\newcommand{\Lam}{\Lambda}  % backward compatibility
\newcommand{\bLa}{{\boldsymbol{\La}}}
\newcommand{\lah}{{\hat{\lam}}}

\newcommand{\bmu}{{\boldsymbol{\mu}}}

\newcommand{\bXi}{{\boldsymbol{\Xi}}}
%\newcommand{\rvx}{{\mathsf{x}}}
%\newcommand{\rvy}{{\mathrm{y}}}
\newcommand{\bPi}{{\boldsymbol{\Pi}}}

\newcommand{\rht}{{\tilde{\rho}}}
\newcommand{\rhc}{{\check{\rho}}}

\newcommand{\bSi}{{\boldsymbol{\Sigma}}}

\newcommand{\ups}{\upsilon}
\newcommand{\Ups}{\Upsilon}
\newcommand{\bUp}{{\boldsymbol{\Ups}}}

\newcommand{\bPs}{{\boldsymbol{\Psi}}}

\newcommand{\w}{\omega}
\newcommand{\wh}{{\hat{\omega}}}
\newcommand{\W}{\Omega}

\newcommand{\dagg}{\dagger}
\newcommand{\dagbh}{{\mathbf{h}}^\dagger}
\newcommand{\dagbH}{{\mathbf{H}}^\dagger}


==> fig/latex_src/def_header.tex <==
% GWW DEFINITIONS AND ABBREVIATIONS

% TeX Defs

                 % subequations environment, etc
%\usepackage{amssymb}  % get, among others, blackboard bold fonts
                      % defines extra symbols like \gtreqless, etc
%\usepackage{verbatim} % get comment environment, + new verbatim
% \usepackage{amsxtra}  % get, eg, \accentedsymbol
%
%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\argsup}{arg\,sup}
%\DeclareMathOperator*{\arginf}{arg\,inf}
%\DeclareMathOperator{\erfc}{erfc}
%\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\cum}{cum}
%\DeclareMathOperator{\sgn}{sgn}
%\DeclareMathOperator{\tr}{tr}
%\DeclareMathOperator{\spn}{span}
%\DeclareMathOperator{\adj}{adj}
%\DeclareMathOperator{\var}{var}
%\DeclareMathOperator{\cov}{cov}
%\DeclareMathOperator{\sech}{sech}
%\DeclareMathOperator{\sinc}{sinc}
%\DeclareMathOperator*{\lms}{l.i.m.\,}
%\newcommand{\varop}[1]{\var\left[{#1}\right]}
%\newcommand{\covop}[2]{\cov\left({#1},{#2}\right)}
%
%\newcommand{\p}{\partial}

% LIST ENVIRONMENTS

\newcounter{actr}
\newenvironment{alist}%
{\begin{list}{(\alph{actr})}{\usecounter{actr}}}{\end{list}}

\newcounter{ictr}
\newenvironment{ilist}%
{\begin{list}{(\roman{ictr})}{\usecounter{ictr}}}{\end{list}}

\iffalse

% SPACING ENVIRONMENTS

\newenvironment{singlespace}%
{\begin{spacing}{1}}{\end{spacing}}

\newenvironment{onehalfspace}% for 11pt font
{\begin{spacing}{1.21}}{\end{spacing}}

\newenvironment{doublespace}% for 11pt font
{\begin{spacing}{1.62}}{\end{spacing}}

\fi

% THEOREM ENVIRONMENTS
\newtheorem{obs}{Observation}
\newtheorem{remark}{Remark}
\newtheorem{thm}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{corol}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{defn}{Definition}
\newtheorem{fact}{Fact}
%\newenvironment{proof}%
%{\noindent{\em Proof: } \begin{singlespace} \small \noindent}%
%{\noindent\qed \end{singlespace}}
\newenvironment{new-proof}[1]
{{\em Proof }:\\}%
{ \noindent\qed }
%
\newcommand{\abs}[1]{\left|#1\right|}
%\newcommand{\comb}[2]{{#1\choose#2}}
\newcommand{\comb}[2]{\binom{#1}{#2}}
\newcommand{\ie}{i.e.}
\newcommand{\eg}{e.g.}
\newcommand{\etc}{etc.}
\newcommand{\viz}{viz.}
\newcommand{\etal}{et al.}
\newcommand{\cf}{cf.}

\newcommand{\vect}[3]{\begin{bmatrix} #1 & #2 & \cdots & #3 \end{bmatrix}^\T}

\newcommand{\dsp}{.5\baselineskip}             % double space amount
\newcommand{\down}{\vspace{\dsp}}              % double space command
\newcommand{\ddown}{\vspace{\baselineskip}}    % quadruple space command
\newcommand{\spec}{\hspace*{1pt}}              % little bit of space
\newcommand{\ds}{\displaystyle}                % abbreviation
\newcommand{\ts}{\textstyle}                % abbreviation
\newcommand{\nin}{\noindent}                   % noindent abbreviation
\newcommand{\cvar}[1]{\mathrm{var_{#1}\,}}
%\newcommand{\qed}{\rule[0.1ex]{1.4ex}{1.6ex}}
\newcommand{\mycap}[2]{\caption{\sl #2 \label{#1}}}
\newcommand{\subcap}[1]{{\begin{center}\sl #1\end{center}}}
\newcommand{\ditem}[1]{\item[#1 \hspace*{\fill}]}
\newcommand{\appfig}{\vspace*{1in}\begin{center} Figure appended to
                       end of manuscript. \end{center} \vspace*{1in}}
\newcommand{\psx}[1]{\centerline{\epsfxsize=6in \epsfbox{#1}}}
\newcommand{\psy}[1]{\centerline{\epsfysize=7in \epsfbox{#1}}}
\newcommand{\psxs}[2]{\centerline{\epsfxsize=#1in \epsfbox{#2}}}
\newcommand{\psxsbb}[3]{\centerline{\epsfxsize=#1in \epsfbox[#3]{#2}}}
\newcommand{\psys}[2]{\centerline{\epsfysize=#1in \epsfbox{#2}}}
\newcommand{\convsamp}[3]{\left.\left\{#1 \ast #2\right\}\right|_{#3}}
\newcommand{\gap}{\qquad}
\newcommand{\order}[1]{\mathcal{O}\left(#1\right)}
\newcommand{\arror}[3]{\begin{cases} #1 & #2 \\
                                     #3 & \text{otherwise} \end{cases}}
\newcommand{\arrorc}[3]{\begin{cases} #1 & #2 \\
                                     #3 & \text{otherwise,} \end{cases}}
\newcommand{\arrorp}[3]{\begin{cases} #1 & #2 \\
                                     #3 & \text{otherwise.} \end{cases}}
\newcommand{\darror}[4]{\begin{cases} #1 & #2 \\ #3 & #4 \end{cases}}
% \newcommand{\defeq}{\stackrel{\triangle}{=}}
\newcommand{\defeq}{\stackrel{\Delta}{=}}
\newcommand{\msconv}{\stackrel{\mathrm{m.s.}}{\longrightarrow}}
\newcommand{\pwaeconv}{\stackrel{\mathrm{p.w.a.e.}}{\longrightarrow}}
\newcommand{\peq}{\stackrel{\mathcal{P}}{=}}
% \newcommand{\glt}{ \begin{array}{c} \Hh=H_1 \\
%  \renewcommand{\arraystretch}{.3}
%  \begin{array}{c} > \\ < \end{array}
%  \renewcommand{\arraystretch}{1} \\ \Hh=H_0 \end{array}}

\hyphenation{or-tho-nor-mal}
\hyphenation{wave-let wave-lets}

\newcommand{\crb}{Cram\'{e}r-Rao}  % obsolete
\newcommand{\CR}{Cram\'{e}r-Rao}
\newcommand{\KL}{Karhunen-Lo\`{e}ve}
\newcommand{\sE}{\sqrt{E_0}}
\newcommand{\pe}{\Pr(\eps)}
\newcommand{\jw}{j\w}
\newcommand{\ejw}{e^{j\w}}
\newcommand{\ejv}{e^{j\nu}}
\newcommand{\wo}{{\w_0}}
\newcommand{\woh}{{\wh_0}}
\newcommand{\sumi}[1]{\sum_{#1=-\infty}^{+\infty}}
\newcommand{\inti}{\int_{-\infty}^{+\infty}}
\newcommand{\intp}{\int_{-\pi}^{\pi}}
\newcommand{\nintp}{\frac{1}{2\pi}\int_{-\pi}^{\pi}}
\newcommand{\inth}{\int_{0}^{\infty}}
\newcommand{\E}[1]{E\left[{#1}\right]}
\newcommand{\bigE}[1]{E\bigl[{#1}\bigr]}
\newcommand{\BigE}[1]{E\Bigl[{#1}\Bigr]}
\newcommand{\biggE}[1]{E\biggl[{#1}\biggr]}
\newcommand{\BiggE}[1]{E\Biggl[{#1}\Biggr]}
\newcommand{\Prob}[1]{\Pr\left[{#1}\right]}
\newcommand{\Pu}[1]{\Pr\left[{#1}\right]} % obsolete; same as \Prob now
\newcommand{\Pc}[2]{\Pr\left[{#1}\mid{#2}\right]}  % obsolete
\newcommand{\Pcb}[2]{\Pr\left[{#1}\Bigm|{#2}\right]} % obsolete
\newcommand{\Q}[1]{\mathcal{Q}\left({#1}\right)}
\newcommand{\FT}[1]{\mathcal{F}\left\{{#1}\right\}}
\newcommand{\LT}[1]{\mathcal{L}\left\{{#1}\right\}}
\newcommand{\ZT}[1]{\mathcal{Z}\left\{{#1}\right\}}
%\newcommand{\reals}{\mathbf{R}}
\newcommand{\reals}{\mathbb{R}}
%\newcommand{\ints}{\mathbf{Z}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\compls}{\mathbb{C}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\rats}{\mathbb{Q}}
\newcommand{\ltwor}{L^2(\reals)}
\newcommand{\ltwoz}{\ell^2(\ints)}
\newcommand{\ltwow}{L^2(\Omega)}
% \newcommand{\ltwo}{\mathbf{L}^2}
% \newcommand{\ltwor}{\mathbf{L}^2 (\reals)}
% \newcommand{\ltwoz}{\mathbf{l}^2 (\ints)}
\newcommand{\sys}[1]{\mathcal{S}\left\{#1\right\}}
\newcommand{\nn}{\nonumber}
\newcommand{\mrm}{\mathrm}
\newcommand{\ip}[2]{\left\langle{#1},{#2}\right\rangle}
\newcommand{\di}[2]{d\left({#1},{#2}\right)}
\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\phase}{\measuredangle}

\newcommand{\Ht}{\mathrm{H}}
\newcommand{\T}{{\mathrm{T}}}
% \newcommand{\R}{\Re\mathit{e}}
% \newcommand{\I}{\Im\mathit{m}}
\DeclareMathOperator{\R}{Re}
\DeclareMathOperator{\I}{Im}


==> fig/latex_src/rv_header.tex <==
\DeclareMathAlphabet{\mathbsf}{OT1}{cmss}{bx}{n}% bold sans serif
\DeclareMathAlphabet{\mathssf}{OT1}{cmss}{m}{sl}% slanted sans serif

% define some useful uppercase Greek letters in regular and bold sf
\DeclareSymbolFont{bsfletters}{OT1}{cmss}{bx}{n}
\DeclareSymbolFont{ssfletters}{OT1}{cmss}{m}{n}
\DeclareMathSymbol{\bsfGamma}{0}{bsfletters}{'000}
\DeclareMathSymbol{\ssfGamma}{0}{ssfletters}{'000}
\DeclareMathSymbol{\bsfDelta}{0}{bsfletters}{'001}
\DeclareMathSymbol{\ssfDelta}{0}{ssfletters}{'001}
\DeclareMathSymbol{\bsfTheta}{0}{bsfletters}{'002}
\DeclareMathSymbol{\ssfTheta}{0}{ssfletters}{'002}
\DeclareMathSymbol{\bsfLambda}{0}{bsfletters}{'003}
\DeclareMathSymbol{\ssfLambda}{0}{ssfletters}{'003}
\DeclareMathSymbol{\bsfXi}{0}{bsfletters}{'004}
\DeclareMathSymbol{\ssfXi}{0}{ssfletters}{'004}
\DeclareMathSymbol{\bsfPi}{0}{bsfletters}{'005}
\DeclareMathSymbol{\ssfPi}{0}{ssfletters}{'005}
\DeclareMathSymbol{\bsfSigma}{0}{bsfletters}{'006}
\DeclareMathSymbol{\ssfSigma}{0}{ssfletters}{'006}
\DeclareMathSymbol{\bsfUpsilon}{0}{bsfletters}{'007}
\DeclareMathSymbol{\ssfUpsilon}{0}{ssfletters}{'007}
\DeclareMathSymbol{\bsfPhi}{0}{bsfletters}{'010}
\DeclareMathSymbol{\ssfPhi}{0}{ssfletters}{'010}
\DeclareMathSymbol{\bsfPsi}{0}{bsfletters}{'011}
\DeclareMathSymbol{\ssfPsi}{0}{ssfletters}{'011}
\DeclareMathSymbol{\bsfOmega}{0}{bsfletters}{'012}
\DeclareMathSymbol{\ssfOmega}{0}{ssfletters}{'012}

\newcommand{\fxfm}{\stackrel{\mathcal{F}}{\longleftrightarrow}}
\newcommand{\lxfm}{\stackrel{\mathcal{L}}{\longleftrightarrow}}
\newcommand{\zxfm}{\stackrel{\mathcal{Z}}{\longleftrightarrow}}

\DeclareMathOperator*{\gltop}{\gtreqless}
\newcommand{\glt}{\;\gltop^{\Hh=\svH_1}_{\Hh=\svH_0}\;}
\newcommand{\glty}{\;\gltop^{\Hh(\svy)=\svH_1}_{\Hh(\svy)=\svH_0}\;}
\newcommand{\gltby}{\;\gltop^{\Hh(\svby)=\svH_1}_{\Hh(\svby)=\svH_0}\;}
\DeclareMathOperator*{\geltop}{\genfrac{}{}{0pt}{}{\ge}{<}}
\newcommand{\gelty}{\;\geltop^{\Hh(\svy)=\svH_1}_{\Hh(\svy)=\svH_0}\;}
\newcommand{\geltby}{\;\geltop^{\Hh(\svby)=\svH_1}_{\Hh(\svby)=\svH_0}\;}
\renewcommand{\pe}{\Pr(e)}
\renewcommand{\defeq}{\triangleq}
\newcommand{\like}{\svlike}
\newcommand{\rvlike}{\mathssf{L}}
\newcommand{\sst}{\cl}
\newcommand{\svlike}{L}
\newcommand{\llike}{\rvllike}
\newcommand{\rvllike}{\cl}
\newcommand{\svllike}{l}
\newcommand{\bllike}{\rvbllike}
\newcommand{\rvbllike}{\boldsymbol{\cl}}
\newcommand{\svbllike}{\mathbf{l}}
\newcommand{\Qb}{\overline{Q}}
\renewcommand{\comb}[2]{\binom{#1}{#2}}


%% Random/sample variable/vector declarations.  Please add in alphabetical
%% order.  First section is for capitals.  Second for lower case.
% Capitals
\newcommand{\rvA}{{\mathssf{A}}}    % A
\newcommand{\svA}{A}
\newcommand{\rvbA}{{\mathbsf{A}}}
\newcommand{\svbA}{{\mathbf{A}}}
\newcommand{\rvD}{{\mathssf{D}}}    % D
\newcommand{\svD}{D}
\newcommand{\rvbD}{{\mathbsf{D}}}
\newcommand{\svbD}{{\mathbf{D}}}
\newcommand{\rvFh}{{\hat{\mathssf{F}}}} % F
\newcommand{\rvF}{{\mathssf{F}}}
\newcommand{\rvHh}{{\hat{\mathssf{H}}}} % H
\newcommand{\rvH}{{\mathssf{H}}}
\newcommand{\svH}{H}
\newcommand{\svHh}{{\hat{\svH}}}
\newcommand{\rvL}{{\mathssf{L}}}    % L
\newcommand{\rvN}{{\mathssf{N}}}    % N
\newcommand{\rvR}{{\mathssf{R}}}    % R
\newcommand{\rvRh}{{\hat{\rvR}}}
\newcommand{\rvS}{{\mathssf{S}}}    % S
\newcommand{\rvSh}{{\hat{\rvS}}}
\newcommand{\rvW}{{\mathssf{W}}}    % W
\newcommand{\rvX}{{\mathssf{X}}}    % X, random variable
\newcommand{\svX}{X}
\newcommand{\rvXt}{{\tilde{\rvX}}}
\newcommand{\rvY}{{\mathssf{Y}}}    % Y
\newcommand{\rvZ}{{\mathssf{Z}}}    % Z

\newcommand{\rva}{{\mathssf{a}}}    % a
\newcommand{\rvah}{{\hat{\rva}}}
\newcommand{\sva}{a}
\newcommand{\svah}{{\hat{\sva}}}
\newcommand{\rvba}{{\mathbsf{a}}}
\newcommand{\svba}{{\mathbf{a}}}
\newcommand{\rvhba}{\hat{{{\mathbsf{{a}}}}}}


\newcommand{\rvb}{{\mathssf{b}}}    % b
\newcommand{\rvbB}{{\mathbsf{B}}}   % b
\newcommand{\rvbb}{{\mathbsf{b}}}
\newcommand{\rvhbb}{\hat{{{\mathbsf{{b}}}}}}
\newcommand{\svbb}{{\mathbf{b}}}

\newcommand{\rvc}{{\mathssf{c}}}    % c
\newcommand{\rvch}{{\hat{\rvc}}}
\newcommand{\svc}{c}
\newcommand{\svch}{{\hat{\svc}}}
\newcommand{\rvbc}{{\mathbsf{c}}}
\newcommand{\svbc}{{\mathbf{c}}}

\newcommand{\rvd}{{\mathssf{d}}}    % d
\newcommand{\rvdh}{{\hat{\rvd}}}
\newcommand{\svd}{d}
\newcommand{\svdh}{{\hat{\svd}}}
\newcommand{\rvbd}{{\mathbsf{d}}}
\newcommand{\svbd}{{\mathbf{d}}}



\newcommand{\rve}{{\mathssf{e}}}    % e
\newcommand{\sve}{e}
\newcommand{\rvbe}{{\mathbsf{e}}}
\newcommand{\svbe}{{\mathbf{e}}}
\newcommand{\rvf}{{\mathssf{f}}}    % f
\newcommand{\rvhf}{{\hat{{\mathssf{f}}}}}    % f

\newcommand{\svf}{f}
\newcommand{\rvbf}{{\mathbsf{f}}}
\newcommand{\svbf}{{\mathbf{f}}}
\newcommand{\rvg}{{\mathssf{g}}}    % g
\newcommand{\svg}{g}
\newcommand{\rvbg}{{\mathbsf{g}}}
\newcommand{\rvbG}{{\mathbsf{G}}}
\newcommand{\svbg}{{\mathbf{g}}}
\newcommand{\rvh}{{\mathssf{h}}}    % h
\newcommand{\svh}{h}
\newcommand{\rvbh}{{\mathbsf{h}}}
\newcommand{\rvbH}{{\mathbsf{H}}}
\newcommand{\svbh}{{\mathbf{h}}}
\newcommand{\rvk}{{\mathssf{k}}}    % k
\newcommand{\rvhk}{{\hat{\mathssf{k}}}}    % k

\newcommand{\svk}{k}
\newcommand{\rvl}{{\mathssf{l}}}    % l

\newcommand{\rvm}{{\mathssf{m}}}    % m
\newcommand{\svm}{m}
\newcommand{\rvbm}{{\mathbsf{m}}}
\newcommand{\svbm}{{\mathbf{m}}}
\newcommand{\rvn}{{\mathssf{n}}}    % n
\newcommand{\rvbn}{{\mathbsf{n}}}
\newcommand{\rvp}{{\mathssf{p}}}    % p
\newcommand{\svp}{p}
\newcommand{\rvq}{{\mathssf{q}}}    % q
\newcommand{\svq}{q}
\newcommand{\svQ}{Q}
\newcommand{\rvr}{{\mathssf{r}}}    % r
\newcommand{\rvbr}{{\mathbsf{r}}}
\newcommand{\svr}{r}
\newcommand{\rvs}{{\mathssf{s}}}    % s
\newcommand{\rvbs}{{\mathbsf{s}}}
\newcommand{\svs}{s}
\newcommand{\svbs}{{\mathbf{s}}}
\newcommand{\rvt}{{\mathssf{t}}}    % t
\newcommand{\rvbt}{{\mathbsf{t}}}
\newcommand{\rvhbt}{\hat{{\mathbsf{t}}}}
\newcommand{\svt}{t}
\newcommand{\svbt}{{\mathbf{t}}}
\newcommand{\rvu}{{\mathssf{u}}}    % u
\newcommand{\svu}{u}
\newcommand{\svuh}{{\hat{\svu}}}
\newcommand{\rvbu}{{\mathbsf{u}}}
\newcommand{\rvbU}{{\mathbsf{U}}}
\newcommand{\svbu}{{\mathbf{u}}}
\newcommand{\rvv}{{\mathssf{v}}}    % v
\newcommand{\svv}{v}
\newcommand{\svvh}{{\hat{\svv}}}
\newcommand{\rvbv}{{\mathbsf{v}}}
\newcommand{\rvbV}{{\mathbsf{V}}}
\newcommand{\svbv}{{\mathbf{v}}}
\newcommand{\rvvh}{{\hat{\rvv}}}
\newcommand{\rvw}{{\mathssf{w}}}    % w
\newcommand{\svw}{w}
\newcommand{\rvwh}{{\hat{\rvw}}}
\newcommand{\svwh}{{\hat{\svw}}}
\newcommand{\rvbw}{{\mathbsf{w}}}
\newcommand{\svbw}{{\mathbf{w}}}
\newcommand{\rvx}{{\mathssf{x}}}    % x, random variable
\newcommand{\rvxh}{{\hat{\rvx}}}
\newcommand{\rvxt}{{\tilde{\rvx}}}
\newcommand{\svx}{x}            % sample value
\newcommand{\svxh}{{\hat{\svx}}}
\newcommand{\svxt}{{\tilde{\svx}}}
\newcommand{\rvbx}{{\mathbsf{x}}}
\newcommand{\rvbxh}{{\hat{\rvbx}}}
\newcommand{\rvbxt}{{\tilde{\rvbx}}}
\newcommand{\svbx}{{\mathbf{\svx}}}
\newcommand{\svbxt}{{\tilde{\svbx}}}
\newcommand{\svbxh}{{\hat{\mathbf{x}}}}
\newcommand{\rvy}{{\mathssf{y}}}    % y
\newcommand{\rvyh}{{\hat{\mathssf{y}}}}
\newcommand{\svy}{y}
\newcommand{\rvyt}{{\tilde{\rvy}}}
\newcommand{\svyt}{{\tilde{\svy}}}
\newcommand{\svyh}{{\hat{\svy}}}
\newcommand{\rvby}{{\mathbsf{y}}}
\newcommand{\rvbyt}{{\tilde{\rvby}}}
\newcommand{\svby}{{\mathbf{y}}}
\newcommand{\svbyt}{{\tilde{\svby}}}
\newcommand{\rvz}{{\mathssf{z}}}    % z
\newcommand{\rvzh}{{\hat{\rvz}}}
\newcommand{\rvzt}{{\tilde{\rvz}}}
\newcommand{\svz}{z}
\newcommand{\svzh}{{\hat{\svz}}}
\newcommand{\rvbz}{{\mathbsf{z}}}
\newcommand{\svbz}{{\mathbf{z}}}

\newcommand{\rvB}{{\mathssf{B}}}
\newcommand{\rvJ}{{\mathssf{J}}}
\newcommand{\rvK}{{\mathssf{K}}}
\newcommand{\rvT}{{\mathssf{T}}}
\newcommand{\rvU}{{\mathssf{U}}}
\newcommand{\rvV}{{\mathssf{V}}}

% Handle uppercase Greek differently
\newcommand{\rvTh}{\ssfTheta}
\newcommand{\svTh}{\Theta}
\newcommand{\rvbTh}{\bsfTheta}
\newcommand{\svbTh}{\boldsymbol{\Theta}}
\newcommand{\rvPh}{\ssfPhi}
\newcommand{\svPh}{\Phi}
\newcommand{\rvbPh}{\bsfPhi}
\newcommand{\svbPh}{\boldsymbol{\Phi}}

\newcommand{\ddx}{\frac{\p}{\p \svx}}
\newcommand{\ddbx}{\frac{\p}{\p\svbx}}

%  --add new macros below this line--

% \newcommand{\iid}{\emph{i.i.d.}}
\newcommand{\iid}{i.i.d.}

\newcommand{\corolref}[1]{Corollary~\mbox{\ref{#1}}}
\newcommand{\thrmref}[1]{Theorem~\mbox{\ref{#1}}}
\newcommand{\lemref}[1]{Lemma~\mbox{\ref{#1}}}
\newcommand{\figref}[1]{Figure~\mbox{\ref{#1}}}
\newcommand{\secref}[1]{Section~\mbox{\ref{#1}}}
\newcommand{\chapref}[1]{Chapter~\mbox{\ref{#1}}}
\newcommand{\appref}[1]{Appendix~\mbox{\ref{#1}}}


==> fig/latex_src/schematicE.tex <==
\begin{pspicture}[showgrid=false](0,-8)(9, 0)
%\begin{pspicture}[showgrid=true](0,-8)(9, 0)
	\psset{gratioWh=2}
%	\pssignal(0,0) {S}{$S^{k}$}
	\pnode(0,0){sdot}
	
	%%%%%%%%%%%%%%%%%%  Encoders %%%%%%%%%%%%%%%%%%

	\newcount\cnt

	\psfblock(1.75,0){enc}{Encoder}
	\dotnode(3.5,0){dot1}
	\dotnode(3.5,-2.5){dot2}
	\dotnode(3.5,-5.6){dotn}	
%	\dotnode(7,0){dot2}
%	\dotnode(1,0){dot3}
%	\dotnode(1,-2.5){dot4}
%	\pscircleop[operation=plus](1,-2.5){op3} 
	
%	\pssignal(3,-2.5){W}{$W^{k}$}
%	\pssignal(1,-3.5) {U}{$U^{k}$}
	
	%%%%%%%%%%%%%%%%%% Multipliers %%%%%%%%%%%%%%%%%%
	\cnt=0
	\psforeach{\ry}{0,-2.5, -5.6}{\advance\cnt by 1\relax
		\pscircleop[operation=times](4.5,\ry){op\the\cnt}
	}
	
	%%%%%%%%%%%%%%%%%%  Decoders %%%%%%%%%%%%%%%%%%
	\psfblock(6.5,0){dec1}{Decoder $1$}
	\psfblock(6.5,-2.5){dec2}{Decoder $2$}
	\psfblock(6.5,-5.6){decn}{Decoder $n$}		
	%%%%%%%%%%%%%%%%%%  S hat %%%%%%%%%%%%%%%%%%
%	\pssignal(14,0){b1}{$\hat{S}_{1}^{m}$}
%	\pssignal(14,-2.5){b2}{$\hat{S}_{2}^{m}$}
	\pnode(8.25,0){s1hatdot}
	\pnode(8.25,-2.5){s2hatdot}
	\pnode(8.25,-5.6){snhatdot}

	%%%%%%%%%%%%%%%%%%  Noise symbols %%%%%%%%%%%%%%%%%%
	% Draw N1 noise symbols
	\pssignal(4.5,-1){N1_1}{$N_{1}^{W}$}
	\pssignal(4.5,-3.5){N2_1}{$N_{2}^{W}$}
	\pssignal(4.5,-6.6){Nn_1}{$N_{n}^{W}$}
		
%	\psldots[angle=90,ldotssep=0.1,ldotssize=.1](4.5,-4.25)
%	\psldots[angle=90,ldotssize=.05](5.5,-4.1)
	\psldots[angle=90,ldotssize=.05](6.5,-4.05)
	
	%%%%%%%%%%%%%%%%%%  Connecting blocks 	%%%%%%%%%%%%%%%%%%
	\nclist[style=Arrow]{ncline}[naput]{sdot,enc $S^{N}$,op1 $X^{W}$,dec1 $Y_{1}^{W}$,s1hatdot $\hat{S}_{1}^{N}$}
	\nclist[style=Arrow]{ncline}[naput]{op2,dec2 $Y_{2}^{W}$,s2hatdot $\hat{S}_{2}^{N}$}
	\nclist[style=Arrow]{ncline}[naput]{op3,decn $Y_{n}^{W}$,snhatdot $\hat{S}_{n}^{N}$}
	\ncangle[style=Arrow,angleA=-90,angleB=180]{dot1}{op2}
	\ncangle[style=Arrow,angleA=-90,angleB=180]{dot2}{op3}
%	\ncangle[style=Arrow,angleA=-90,angleB=180]{dotn}{op3}
	\ncline[style=Arrow]{N1_1}{op1}
	\ncline[style=Arrow]{N2_1}{op2}
	\ncline[style=Arrow]{Nn_1}{op3}
%	\ncline[style=Arrow]{W}{op3}
%	\ncline[style=Arrow]{dotn}{op3}
%	\ncline[style=Arrow]{op3}{U}
	
\end{pspicture}

==> fig/latex_src/schematicE_blocks.tex <==
\begin{pspicture}[showgrid=false](0,-8)(9, 0)
%\begin{pspicture}[showgrid=true](0,-8)(9, 0)
	\psset{gratioWh=2}
%	\pssignal(0,0) {S}{$S^{k}$}
	\pnode(0,0){sdot}
	
	%%%%%%%%%%%%%%%%%%  Encoders %%%%%%%%%%%%%%%%%%

	\newcount\cnt
	\psfblock(1.75,0){enc}{Encoder}
	\dotnode(3.1,0){dot1}
	\dotnode(3.1,-2.5){dot2}
	\dotnode(3.1,-5.6){dotn}	
%	\dotnode(7,0){dot2}
%	\dotnode(1,0){dot3}
%	\dotnode(1,-2.5){dot4}
%	\pscircleop[operation=plus](1,-2.5){op3} 
	
%	\pssignal(3,-2.5){W}{$W^{k}$}
%	\pssignal(1,-3.5) {U}{$U^{k}$}
	
	%%%%%%%%%%%%%%%%%% Multipliers %%%%%%%%%%%%%%%%%%
%	\cnt=0
%	\psforeach{\ry}{0,-2.5, -5.6}{\advance\cnt by 1\relax
%		\pscircleop[operation=times](4.5,\ry){op\the\cnt}
%	}
	
	%%%%%%%%%%%%%%%%%%  Decoders %%%%%%%%%%%%%%%%%%
%	\psfblock(7.75,0){dec1}{Decoder $1$}
%	\psfblock(7.75,-2.5){dec2}{Decoder $2$}
%	\psfblock(7.75,-5.6){decn}{Decoder $n$}
	\psfblock(7.25,0){dec1}{Decoder $1$}
	\psfblock(7.25,-2.5){dec2}{Decoder $2$}
	\psfblock(7.25,-5.6){decn}{Decoder $K$}

%	\psfblock(6.5,-2.5){dec2}{Decoder $2$}
%	\psfblock(6.5,-5.6){decn}{Decoder $n$}		
	%%%%%%%%%%%%%%%%%%  S hat %%%%%%%%%%%%%%%%%%
%	\pssignal(14,0){b1}{$\hat{S}_{1}^{m}$}
%	\pssignal(14,-2.5){b2}{$\hat{S}_{2}^{m}$}
	\pnode(9,0){s1hatdot}
	\pnode(9,-2.5){s2hatdot}
	\pnode(9,-5.6){snhatdot}
%	\pnode(8.25,-2.5){s2hatdot}
%	\pnode(8.25,-5.6){snhatdot}

	%%%%%%%%%%%%%%%%%%  Noise symbols %%%%%%%%%%%%%%%%%%
	% Draw N1 noise symbols
%	\pssignal(4.5,-1){N1_1}{$N_{1}^{W}$}
%	\pssignal(4.5,-3.5){N2_1}{$N_{2}^{W}$}
%	\pssignal(4.5,-6.6){Nn_1}{$N_{n}^{W}$}

%	\psfblock(5,0){BEC1}{$\operatorname{BEC}(\epsilon_1)$}
	\psfblock(4.5,0){BEC1}{$\operatorname{BEC}(\epsilon_1)$}	
	\psfblock(4.5,-2.5){BEC2}{$\operatorname{BEC}(\epsilon_2)$}
	\psfblock(4.5,-5.6){BECn}{$\operatorname{BEC}(\epsilon_K)$}
		
%	\psldots[angle=90,ldotssep=0.1,ldotssize=.1](4.5,-4.25)
%	\psldots[angle=90,ldotssize=.05](5.5,-4.1)
	\psldots[angle=90,ldotssize=.05](7.25,-4.05)
	
	%%%%%%%%%%%%%%%%%%  Connecting blocks 	%%%%%%%%%%%%%%%%%%
%	\nclist[style=Arrow]{ncline}[naput]{sdot,enc $S^{N}$,op1 $X^{W}$,dec1 $Y_{1}^{W}$,s1hatdot $\hat{S}_{1}^{N}$}
%	\nclist[style=Arrow]{ncline}[naput]{op2,dec2 $Y_{2}^{W}$,s2hatdot $\hat{S}_{2}^{N}$}
%	\nclist[style=Arrow]{ncline}[naput]{op3,decn $Y_{n}^{W}$,snhatdot $\hat{S}_{n}^{N}$}
	\nclist[style=Arrow]{ncline}[naput]{sdot,enc $S^{N}$,BEC1 $X^{W}$,dec1 $Y_{1}^{W}$,s1hatdot $\hat{S}_{1}^{N}$}
	\nclist[style=Arrow]{ncline}[naput]{BEC2,dec2 $Y_{2}^{W}$,s2hatdot $\hat{S}_{2}^{N}$}
	\nclist[style=Arrow]{ncline}[naput]{BECn,decn $Y_{n}^{W}$,snhatdot $\hat{S}_{n}^{N}$}
	\ncangle[style=Arrow,angleA=-90,angleB=180]{dot1}{BEC2}
	\ncangle[style=Arrow,angleA=-90,angleB=180]{dot2}{BECn}
%	\ncangle[style=Arrow,angleA=-90,angleB=180]{dotn}{op3}
%	\ncline[style=Arrow]{N1_1}{op1}
%	\ncline[style=Arrow]{N2_1}{op2}
%	\ncline[style=Arrow]{Nn_1}{op3}
%	\ncline[style=Arrow]{W}{op3}
%	\ncline[style=Arrow]{dotn}{op3}
%	\ncline[style=Arrow]{op3}{U}
	
\end{pspicture}

==> fig/latex_src/schematicE_blocks_arrow.tex <==
\begin{pspicture}[showgrid=false](0,-8)(9, 0)
%\begin{pspicture}[showgrid=true](0,-8)(9, 0)
	\psset{gratioWh=2}
	\pssignal(0,0) {S}{$S^{N}$}
	\pnode(0,0){sdot}
	
	%%%%%%%%%%%%%%%%%%  Encoders %%%%%%%%%%%%%%%%%%

	\newcount\cnt

	\psfblock(1.75,0){enc}{Encoder}
	\dotnode(3.1,0){dot1}
	\dotnode(3.1,-2.5){dot2}
	\dotnode(3.1,-5.6){dotn}	
%	\dotnode(7,0){dot2}
%	\dotnode(1,0){dot3}
%	\dotnode(1,-2.5){dot4}
%	\pscircleop[operation=plus](1,-2.5){op3} 
	
%	\pssignal(3,-2.5){W}{$W^{k}$}
%	\pssignal(1,-3.5) {U}{$U^{k}$}
	
	%%%%%%%%%%%%%%%%%% Multipliers %%%%%%%%%%%%%%%%%%
%	\cnt=0
%	\psforeach{\ry}{0,-2.5, -5.6}{\advance\cnt by 1\relax
%		\pscircleop[operation=times](4.5,\ry){op\the\cnt}
%	}
	
	%%%%%%%%%%%%%%%%%%  Decoders %%%%%%%%%%%%%%%%%%
%	\psfblock(7.75,0){dec1}{Decoder $1$}
%	\psfblock(7.75,-2.5){dec2}{Decoder $2$}
%	\psfblock(7.75,-5.6){decn}{Decoder $n$}
	\psfblock(7.25,0){dec1}{Decoder $1$}
	\psfblock(7.25,-2.5){dec2}{Decoder $2$}
	\psfblock(7.25,-5.6){decn}{Decoder $n$}

%	\psfblock(6.5,-2.5){dec2}{Decoder $2$}
%	\psfblock(6.5,-5.6){decn}{Decoder $n$}		
	%%%%%%%%%%%%%%%%%%  S hat %%%%%%%%%%%%%%%%%%
%	\pssignal(14,0){b1}{$\hat{S}_{1}^{m}$}
%	\pssignal(14,-2.5){b2}{$\hat{S}_{2}^{m}$}
	\pnode(9,0){s1hatdot}
	\pnode(9,-2.5){s2hatdot}
	\pnode(9,-5.6){snhatdot}
	\pssignal(9,0) {S1}{$\hat{S}_{1}^{N}$}
	\pssignal(9,-2.5) {S2}{$\hat{S}_{2}^{N}$}
	\pssignal(9,-5.6) {Sn}{$\hat{S}_{n}^{N}$}			
%	\pnode(8.25,-2.5){s2hatdot}
%	\pnode(8.25,-5.6){snhatdot}

	%%%%%%%%%%%%%%%%%%  Noise symbols %%%%%%%%%%%%%%%%%%
	% Draw N1 noise symbols
%	\pssignal(4.5,-1){N1_1}{$N_{1}^{W}$}
%	\pssignal(4.5,-3.5){N2_1}{$N_{2}^{W}$}
%	\pssignal(4.5,-6.6){Nn_1}{$N_{n}^{W}$}

%	\psfblock(5,0){BEC1}{$\operatorname{BEC}(\epsilon_1)$}
	\psfblock(4.5,0){BEC1}{$\operatorname{BEC}(\epsilon_1)$}	
	\psfblock(4.5,-2.5){BEC2}{$\operatorname{BEC}(\epsilon_2)$}
	\psfblock(4.5,-5.6){BECn}{$\operatorname{BEC}(\epsilon_n)$}
		
%	\psldots[angle=90,ldotssep=0.1,ldotssize=.1](4.5,-4.25)
%	\psldots[angle=90,ldotssize=.05](5.5,-4.1)
	\psldots[angle=90,ldotssize=.05](7.25,-4.05)
	
	%%%%%%%%%%%%%%%%%%  Connecting blocks 	%%%%%%%%%%%%%%%%%%
%	\nclist[style=Arrow]{ncline}[naput]{sdot,enc $S^{N}$,op1 $X^{W}$,dec1 $Y_{1}^{W}$,s1hatdot $\hat{S}_{1}^{N}$}
%	\nclist[style=Arrow]{ncline}[naput]{op2,dec2 $Y_{2}^{W}$,s2hatdot $\hat{S}_{2}^{N}$}
%	\nclist[style=Arrow]{ncline}[naput]{op3,decn $Y_{n}^{W}$,snhatdot $\hat{S}_{n}^{N}$}
%	\nclist[style=Arrow]{ncline}[naput]{sdot,enc $S^{N}$,BEC1 $X^{W}$,dec1 $Y_{1}^{W}$,s1hatdot $\hat{S}_{1}^{N}$}
	\nclist[style=Arrow]{ncline}[naput]{S,enc} 
%	\nclist[style=Arrow]{ncline}[naput]{enc,BEC1 $X^{W}$,dec1 $Y_{1}^{W}$,s1hatdot $\hat{S}_{1}^{N}$}
%	\nclist[style=Arrow]{ncline}[naput]{BEC2,dec2 $Y_{2}^{W}$,s2hatdot $\hat{S}_{2}^{N}$}
%	\nclist[style=Arrow]{ncline}[naput]{BECn,decn $Y_{n}^{W}$,snhatdot $\hat{S}_{n}^{N}$}
	\nclist[style=Arrow]{ncline}[naput]{enc,BEC1 $X^{W}$,dec1 $Y_{1}^{W}$,S1}
	\nclist[style=Arrow]{ncline}[naput]{BEC2,dec2 $Y_{2}^{W}$,S2}
	\nclist[style=Arrow]{ncline}[naput]{BECn,decn $Y_{n}^{W}$,Sn}
	\ncangle[style=Arrow,angleA=-90,angleB=180]{dot1}{BEC2}
	\ncangle[style=Arrow,angleA=-90,angleB=180]{dot2}{BECn}
%	\ncangle[style=Arrow,angleA=-90,angleB=180]{dotn}{op3}
%	\ncline[style=Arrow]{N1_1}{op1}
%	\ncline[style=Arrow]{N2_1}{op2}
%	\ncline[style=Arrow]{Nn_1}{op3}
%	\ncline[style=Arrow]{W}{op3}
%	\ncline[style=Arrow]{dotn}{op3}
%	\ncline[style=Arrow]{op3}{U}
	
\end{pspicture}

==> fig/latex_src/schematicE_two_bec.tex <==
\begin{pspicture}[showgrid=false](0,-8)(9, 0)
%\begin{pspicture}[showgrid=true](0,-8)(9, 0)
	\psset{gratioWh=2}
%	\pssignal(0,0) {S}{$S^{k}$}
	\pnode(0,0){sdot}
	
	%%%%%%%%%%%%%%%%%%  Encoders %%%%%%%%%%%%%%%%%%

	\newcount\cnt
	\psfblock(1.75,0){enc}{Encoder}
	\dotnode(3.1,0){dot1}
	\dotnode(3.1,-2.5){dot2}
%	\dotnode(3.1,-5.6){dotn}	
%	\dotnode(7,0){dot2}
%	\dotnode(1,0){dot3}
%	\dotnode(1,-2.5){dot4}
%	\pscircleop[operation=plus](1,-2.5){op3} 
	
%	\pssignal(3,-2.5){W}{$W^{k}$}
%	\pssignal(1,-3.5) {U}{$U^{k}$}
	
	%%%%%%%%%%%%%%%%%% Multipliers %%%%%%%%%%%%%%%%%%
%	\cnt=0
%	\psforeach{\ry}{0,-2.5, -5.6}{\advance\cnt by 1\relax
%		\pscircleop[operation=times](4.5,\ry){op\the\cnt}
%	}
	
	%%%%%%%%%%%%%%%%%%  Decoders %%%%%%%%%%%%%%%%%%
%	\psfblock(7.75,0){dec1}{Decoder $1$}
%	\psfblock(7.75,-2.5){dec2}{Decoder $2$}
%	\psfblock(7.75,-5.6){decn}{Decoder $n$}
	\psfblock(7.25,0){dec1}{Decoder $1$}
	\psfblock(7.25,-2.5){dec2}{Decoder $2$}
%	\psfblock(7.25,-5.6){decn}{Decoder $K$}

%	\psfblock(6.5,-2.5){dec2}{Decoder $2$}
%	\psfblock(6.5,-5.6){decn}{Decoder $n$}		
	%%%%%%%%%%%%%%%%%%  S hat %%%%%%%%%%%%%%%%%%
%	\pssignal(14,0){b1}{$\hat{S}_{1}^{m}$}
%	\pssignal(14,-2.5){b2}{$\hat{S}_{2}^{m}$}
	\pnode(9,0){s1hatdot}
	\pnode(9,-2.5){s2hatdot}
%	\pnode(9,-5.6){snhatdot}
%	\pnode(8.25,-2.5){s2hatdot}
%	\pnode(8.25,-5.6){snhatdot}

	%%%%%%%%%%%%%%%%%%  Noise symbols %%%%%%%%%%%%%%%%%%
	% Draw N1 noise symbols
%	\pssignal(4.5,-1){N1_1}{$N_{1}^{W}$}
%	\pssignal(4.5,-3.5){N2_1}{$N_{2}^{W}$}
%	\pssignal(4.5,-6.6){Nn_1}{$N_{n}^{W}$}

%	\psfblock(5,0){BEC1}{$\operatorname{BEC}(\epsilon_1)$}
	\psfblock(4.5,0){BEC1}{$\operatorname{BEC}(\epsilon_1)$}	
	\psfblock(4.5,-2.5){BEC2}{$\operatorname{BEC}(\epsilon_2)$}
%	\psfblock(4.5,-5.6){BECn}{$\operatorname{BEC}(\epsilon_K)$}
		
%	\psldots[angle=90,ldotssep=0.1,ldotssize=.1](4.5,-4.25)
%	\psldots[angle=90,ldotssize=.05](5.5,-4.1)
%	\psldots[angle=90,ldotssize=.05](7.25,-4.05)
	
	%%%%%%%%%%%%%%%%%%  Connecting blocks 	%%%%%%%%%%%%%%%%%%
%	\nclist[style=Arrow]{ncline}[naput]{sdot,enc $S^{N}$,op1 $X^{W}$,dec1 $Y_{1}^{W}$,s1hatdot $\hat{S}_{1}^{N}$}
%	\nclist[style=Arrow]{ncline}[naput]{op2,dec2 $Y_{2}^{W}$,s2hatdot $\hat{S}_{2}^{N}$}
%	\nclist[style=Arrow]{ncline}[naput]{op3,decn $Y_{n}^{W}$,snhatdot $\hat{S}_{n}^{N}$}
	\nclist[style=Arrow]{ncline}[naput]{sdot,enc $S^{m}$,BEC1 $X^{n}$,dec1 $Y_{1}^{n}$,s1hatdot $\hat{S}_{1}^{m}$}
	\nclist[style=Arrow]{ncline}[naput]{BEC2,dec2 $Y_{2}^{n}$,s2hatdot $\hat{S}_{2}^{m}$}
%	\nclist[style=Arrow]{ncline}[naput]{BECn,decn $Y_{n}^{W}$,snhatdot $\hat{S}_{n}^{N}$}
	\ncangle[style=Arrow,angleA=-90,angleB=180]{dot1}{BEC2}
%	\ncangle[style=Arrow,angleA=-90,angleB=180]{dot2}{BECn}
%	\ncangle[style=Arrow,angleA=-90,angleB=180]{dotn}{op3}
%	\ncline[style=Arrow]{N1_1}{op1}
%	\ncline[style=Arrow]{N2_1}{op2}
%	\ncline[style=Arrow]{Nn_1}{op3}
%	\ncline[style=Arrow]{W}{op3}
%	\ncline[style=Arrow]{dotn}{op3}
%	\ncline[style=Arrow]{op3}{U}
	
\end{pspicture}

==> latexpand <==
#!/usr/bin/perl
# Inspired by latexpand by D. Musliner, University of Michigan
# 2012, 2013, 2014, 2015: Matthieu Moy <Matthieu.Moy@imag.fr>
# BSD License

use strict;
use Cwd;
use Getopt::Long;
use Pod::Usage;
use IO::Handle;

my $TEXINPUTS = $ENV{'TEXINPUTS'};
if (!$TEXINPUTS) { $TEXINPUTS = getcwd(); }

my $verbose;
my $keep_comments;
my $keep_includes;
my $empty_comments;
my $help;
my $long_help;
my $output;
my $explain;
my $show_graphics;
my $graphics_extensions = ":.pdf:.png:.jpg:.eps";
my $expand_usepackage;
my $expand_bbl;
my $fatal;
my $version;
my $makeatletter;

GetOptions (
	'h' => \$help,
	'help' => \$long_help,
	'verbose|v' => \$verbose,
	'keep-comments' => \$keep_comments,
	'keep-includes' => \$keep_includes,
	'empty-comments' => \$empty_comments,
	'output|o=s' => \$output,
	'explain' => \$explain,
	'show-graphics' => \$show_graphics,
	'graphics-extensions' => \$graphics_extensions,
	'expand-usepackage' => \$expand_usepackage,
	'expand-bbl=s' => \$expand_bbl,
	'fatal' => \$fatal,
	'version' => \$version,
        'makeatletter' => \$makeatletter,
) or pod2usage(2);
version() if $version;
pod2usage(1) if $help;
pod2usage(-exitstatus => 0, -verbose => 2) if $long_help;

sub get_version
{
	# $VERSION's value will be substituted by 'make dist', but the
	# next line won't (the string has to be broken to avoid it).
	my $VERSION = 'v1.2-1-g47e2cee';
	if ($VERSION eq '@LATEXPAND' . '_VERSION@') {
		my($vol,$dir,$file) = File::Spec->splitpath($0);
		chdir($dir);
		$VERSION = `git describe --tags HEAD 2>/dev/null`;
	}
	if ($VERSION eq '') {
		$VERSION = '<unknown version>';
	}
	$VERSION =~ s/^\s+|\s+$//g;
	return $VERSION;
}

sub version
{
	print "latexpand version ". get_version() .".\n";
	exit(0);
}

my $nl = "";
if ($empty_comments) {
	$nl = "%\n";
}

if ($output && $output ne "-") {
	open OUTPUT, '>', "$output" or die $!;
	STDOUT->fdopen(\*OUTPUT, 'w') or die $!;
}

sub say
{
	if ($verbose) {
		print STDERR "$_[0]";
	}
}

my $makeatletter_found;
my $in_preamble;

foreach my $file (@ARGV)
{
	say "processing $file\n";
	$makeatletter_found = 0;
	$in_preamble = 1;
	process_file($file, "  ");
}

sub process_file
{
	my $file = shift;
	my $prefix = (shift || "");
	my $in_comment = 0;
	local(*FILE);
	open(FILE, $file) or die "could not open input file '$file'\n";
	while (my $line = <FILE>) {
		if ($line =~ /^[ \t]*\\endinput/) {
			$line =~ s/(\\endinput.*)\n/% $1/;
			$in_comment = 1;
			process_line($line, $prefix);
			last;
		}
		process_line($line, $prefix, $file);
		if ($line =~ /^%.*[^\n]\z/ || $line =~ /[^\\]%.*[^\n]\z/) {
			# file ends with a comment not ending with a newline
			print "\n";
		}
		# Garbage at end of line after \end{document} is
		# ignored by LaTeX, but we don't allow anything before
		# to avoid e.g. \verb|\end{document}| from terminating
		# the file.
		if (!$keep_comments && $line =~ /^[ \t]*\\end{document}/) {
			last;
		}
	}
	close(FILE);
	return $in_comment;
}

sub process_line
{
	my ($_, $prefix, $file) = @_;
	# Consider \makeatletter only in preamble, because we do want
	# to warn on \someCommand{\makeatletter\command@with@arobase}.
	if ($in_preamble && /^[^%]*\\makeatletter/) {
		$makeatletter_found = 1;
	}
	if ($in_preamble && /^[^%]*\\makeatother/) {
		$makeatletter_found = 0;
	}
	if (!$makeatletter && !$makeatletter_found
	    && (my ($command) = /^[^%]*(\\[[:alpha:]]*@[[:alpha:]]*)/)) {
		print STDERR "Warning: command $command containing @ found in\n";
		print STDERR "Warning: $file.\n";
		print STDERR "Warning: consider using --makeatletter if the result is not compilable.\n";
	}
	unless ($keep_comments) {
		if ($empty_comments) {
			s/^%.*$/%/;
			s/([^\\])%.*$/$1%/;
		} else {
			s/^%.*\n//;
			s/([^\\])%.*\n/$1/;
		}
	}

	unless ($keep_includes) {
		if (my ($before, $ignored, $full_filename, $after)
		    = /^(([^%]|[^\\]%)*)\\include[{\s]+(.*?)[\s}](.*)$/) {
			$full_filename = find_tex_file($full_filename . ".tex");
			if ($full_filename) {
				say $prefix . "Found include for file: $full_filename\n";
				print $before . $nl;
				print '\clearpage{}' . $nl;
				print "% start include $full_filename\n" if ($explain);
				my $in_comment = process_file($full_filename, $prefix . "  ");
				if ($explain) {
				    print " % end include $full_filename\n";
				} elsif ($in_comment) {
				    print "\n";
				}
				print '\clearpage{}' . $nl;
				print $nl . $after . "\n";
				$_ = "";
			}
		} elsif (my ($before, $ignored, $full_filename, $after)
			 = /^(([^%]|[^\\]%)*)\\input[{\s]+(.*?)[\s}](.*)$/) {
			$full_filename = find_tex_file($full_filename, ":.tex");
			if ($full_filename) {
				say $prefix . "Found input for file: $full_filename\n";
				print $before . $nl;
				print "% start input $full_filename\n" if ($explain);
				my $in_comment = process_file($full_filename, $prefix . "  ");
				if ($explain) {
				    print " % end input $full_filename\n";
				} elsif ($in_comment) {
				    print "\n";
				}
				if ($after =~ /[^\s]/) {
				    # LaTeX produces this space, so let's do it also
				    print " " . $nl . $after . "\n";
				} else {
				    print " ";
				}
				$_ = "";
			}
		}
	}
	if ($expand_usepackage) {
		# Don't bother with before and after text, we just require the
		# usepackage to be alone on its line.
		if (my ($package_name) = /^\s*\\usepackage{([^}]*)}\s*(%.*)?$/) {
			my $full = find_file($package_name . ".sty", $TEXINPUTS);
			if ($full) {
				say $prefix . "Found package file: $full\n";
				process_file($full, $prefix . "  ");
				$_ = "";
			} else {
				say $prefix . "Not including external package $package_name\n";
			}
		}
	}
	if ($expand_bbl) {
		if (my ($before, $bib_name, $after)
			 = /^(.*)\\bibliography{([^}]*)}(.*)$/) {
			# The BBL file is not necessarily $bib_name.
			# Take it from the command-line.
			print $before . $nl;
			say $prefix . "Expanding BBL file: $expand_bbl\n";
			process_file($expand_bbl, $prefix . "  ");
			print " " . $nl . $after . "\n";
			$_ = "";
		}
	}
	if ($show_graphics) {
		if (/\\includegraphics(\[[^\]]*\])?{([^}]*)}/) {
			my $full = find_tex_file($2, $graphics_extensions);
			say $prefix . "needs graphics file: ";
			print STDERR "$full\n";
		}
	}
	if (/^[ \t]*\\begin{document}/) {
		$in_preamble = 0;
		if ($makeatletter) {
			print '\makeatletter' . $nl;
		}
	}
	print;
}

# search $1 in $TEXINPUTS, with possible extensions in $2
sub find_tex_file
{
	my $file = shift;
	my $extensions = (shift || ":");
	foreach my $ext (split(':', $extensions, -1)) {
		my $full = find_file($file . $ext, $TEXINPUTS);
		if ($full) {
			return $full;
		}
	}
	if ($fatal) {
		die "ERROR: Could not find file [$file]\n";
	} else {
		print STDERR "Warning: Could not find file [$file]\n";
		return undef;
	}
}

sub find_file
{
	my ($file, $path) = @_;
	if (File::Spec->file_name_is_absolute($file)) {
		if (-e "$file" && ! -d "$file") {
			return $file;
		} else {
			return;
		}
	}
	foreach my $dir (split(':', $path)) {
		if (-e "$dir/$file" && ! -d "$dir/$file") {
			return("$dir/$file");
		}
	}
	return;
}


__END__

=head1 NAME

latexpand - Flatten LaTeX file by expanding \include and \input, ... and  remove comments

=head1 SYNOPSIS

latexpand [options] FILE...

=head2 Options:

	--verbose        show what's going on
	--keep-comments  don't strip comments (comments are lines
                         starting with %, and anything below
                         \end{document})
	--empty-comments keep empty comments (i.e. % at end of lines) for clarity
	--keep-includes  don't expand \input and \include directives
	--expand-usepackage
	                 Expand \usepackage{...} directives if the
	                 corresponding .sty file is found in
	                 $TEXINPUTS (or the current directory if
	                 $TEXINPUTS is not set)
	--expand-bbl FILE
	                 Expand the bibliography by inlining FILE
	                 (should be a *.bbl file)
	--help           this help message
	--output <file>, -o <file>
	                 generate output in <file>
	--explain        generate explanatory comments in output
	--show-graphics  show included graphics
	--graphics_extensions
	                 colon-separated list of possible graphics extensions
	                 (used by --show-graphics to find the actual graphics files)
	--fatal          Die in case a file can't be found.
	--makeatletter   Insert a \makeatletter in the preamble. In some
	                 rare cases it may break your document, but it
	                 may help fixing bad interactions between
	                 @-commands and inclusion (see BUGS section).

=head1 USES

The most common use of latexpand is to simplify distribution of source
LaTeX files, typically to satisfy the requirement of editors and
archival sites (springer, arXiv.org, ...) who force the authors to
submit sources. One does not necessarily want to submit sources with
comments, and uploading a document made of several files including
each other is a bit painful. By default, latexpand answers both
problems by outputing a single LaTeX file that contain no comment.

=head1 GETTING LATEXPAND

The latest version of latexpand is available here:

  https://gitorious.org/latexpand

Versions are uploaded to ctan.org from time to time:

  http://www.ctan.org/pkg/latexpand

=head1 BUGS

Please, report bugs to Matthieu Moy <Matthieu.Moy@imag.fr>.

=head2 Known bugs

=head3 Verbatim

latexpand currently ignores \begin{verbatim} ... \end{verbatim}, and
will therefore process any \include, \input, ... directives that
appear within verbatim environments (while it shouldn't).

=head3 Comment environment

It would be nice to remove code between \begin{comment} and
\end{comment} too if \usepackage{comment} is used.

Code like

	foo%
	\begin{comment}

will produce the incorrect

	foo\begin{comment}

A workaround is to use --empty-comments when such tricky usage of the
comments package is done.

=head3 \makeatletter and use with transfig/xfig with \scalebox{}

If \input{} or \include{} appears as argument to a command, and the
file included contains \makeatletter, then after expansion, the
\makeatletter and the @-command appear as argument to the command,
which is forbidden because the argument is parsed (and the @-command
badly tokenized) before being executed.

This happens with

	\scalebox{ \input{file-generated-by-xfig.pdf_t} }

Workaround: add \makeatletter before the scalebox manually in your
code, like

        \makeatletter{}
	\scalebox{ \input{file-generated-by-xfig.pdf_t} }
        \makeatother{}

In the case of xfig generated files, it is necessary only for the
first occurence.

A more brute-force workaround is to use latexpand --makeatletter.

=head1 SEE ALSO

Instructions to include only the relevant .bib items (french):

https://lacl.fr/~caubert/notes/portabilite-du-tex.html#dependances

=head1 VERSION

This is latexpand version v1.2-1-g47e2cee.


==> one_sided.tex <==
\section{Source-broadcast with One-sided Feedback}
\label{sec:one_sided_feedback}

In this section we consider a one-sided-feedback variation of the problem in Section~\ref{sec:two_users} whereby in a broadcast network with two receivers, a feedback channel is available to only the stronger user.  In this scenario, we show that given the distortion constraints of both users, there is no overhead in the minmax latency achieved.  Specifically, for $i \in \{1, 2\}$, let $\wid$ be the point-to-point optimal latency for user~$i$ and let $\wplusd$ be the Shannon lower bound for the minmax latency where

\begin{align}
\label{eq:wid_optimal}
	\wid = \frac{1 - d_i}{1 - \epsilon_i},
\end{align}
and
\begin{align}
\label{eq:wplusd}
	\wplusd = \max_{i \in \{1, 2\}} \frac{1 - d_i}{1 - \epsilon_i}.
\end{align}
Section~\ref{sec:two_users} showed that for $i \in \{1, 2\}$, user~$i$ can achieve distortion $d_i$ at the optimal latency $\wid$ when a feedback channel is available to \emph{both} users (c.f.\ Section~\ref{sec:individual_latencies} on individual decoding delays).  Clearly, the optimal minmax system latency $\wplusd$ is also achievable in this case.  In contrast, in this section we show that when a feedback channel is available to \emph{only the stronger user}, while the \emph{individual} optimal latencies may or may not be achievable, the overall system latency $\wplusd$ is still achievable.

% achieve point-to-point optimal performance when a feedback channel is available to \emph{both} receivers, in this section we show that point-to-point optimal performance may also be achieved if \emph{only the stronger user} has a feedback channel available.

\input{3/one_sided/problem_formulation}
\input{3/one_sided/one_sided_coding}
\input{3/one_sided/one_sided_optimality}



==> one_sided/fig/indep/d1_big_fig_tab_indep.tex <==
% -------------------------------------------------------------
% d_1 > 
% -------------------------------------------------------------
\begin{figure}
	\centering
%	\includegraphics[scale=0.8]{3/one_sided/fig/system_model_one_sided}
	\includegraphics[scale=1]{3/one_sided/fig/regions_d1_big}
%%	\includegraphics[width=0.6\textwidth]{outer_bound.png}
	\caption{The different regions requiring separate coding schemes when $\epsilon_1^2\epsilon_2 \leq d_1 < \epsilon_1$.}
	\label{fig:regions_d1_big}
\end{figure}

\begin{table}
	\begin{center}
		\begin{tabular}{| c | c |}
%    \caption{The justification for the ordering}
			\hline
			\multicolumn{2}{|c|}{{\bf Ordering of Boundaries for $\depstwo$ when $\epsilon_1^2\epsilon_2 \leq d_1 < \epsilon_1$}} \\
			\hline
			{\bf Inequality} & {\bf Justification}   \\ \hline
			$d_1 < \astar$ & $d_1 < \epsilon_1$ \\ \hline 
			$\astar < d_1/\epsilon_1$ & $d_1 \geq \epsilon_1^2\epsilon_2$ \\ \hline 
			$d_1/\epsilon_1 < \bstar$ &$d_1 < \epsilon_1$ \\ \hline 
			$\bstar < 1$ & $d_1 < \epsilon_1$ \\
			\hline
		\end{tabular}
	\end{center}
	\caption{We justify the ordering of the region boundaries of Figure~\ref{fig:regions_d1_big} when $\epsilon_1^2\epsilon_2 \leq d_1 < \epsilon_1$.  In the left column, we have the ordering between two boundary points, and in the right column, we show the necessary and sufficient condition that justifies the ordering.}	
	\label{tab:d1_big}	
\end{table}

==> one_sided/fig/indep/d1_mid_fig_tab_indep.tex <==
% -------------------------------------------------------------
% < d_1 < 
% -------------------------------------------------------------
\begin{figure}
	\centering
%	\includegraphics[scale=0.8]{3/one_sided/fig/system_model_one_sided}
	\includegraphics[scale=1]{3/one_sided/fig/regions_d1_mid}
%%	\includegraphics[width=0.6\textwidth]{outer_bound.png}
	\caption{The different regions requiring separate coding schemes when $2(\epsilon_1\epsilon_2 - 1)/\epsilon_2 < d_1 < \epsilon_1^2\epsilon_2$.}
	\label{fig:regions_d1_mid}
\end{figure}

\begin{table}
	\begin{center}
		\begin{tabular}{| c | c |}
%    \caption{The justification for the ordering}
			\hline
			\multicolumn{2}{|c|}{{\bf Ordering of Boundaries for $\depstwo$ when $2(\epsilon_1\epsilon_2 - 1)/\epsilon_2 < d_1 < \epsilon_1^2\epsilon_2$}} \\
			\hline
			{\bf Inequality} & {\bf Justification}   \\ \hline
			$d_1 < d_1/\epsilon_1$ & $\epsilon_1 < 1$ \\ \hline 
			$d_1/\epsilon_1 < \astar $ & $d_1 < \epsilon_1^2\epsilon_2$ \\ \hline 
			$\astar < d_1 + (1 - \epsilon_1)$ & $d_1 > 2(\epsilon_1\epsilon_2 - 1)/\epsilon_2$ \\ \hline 			
			$d_1 + (1 - \epsilon_1) < \bstar$ & $d_1 < \epsilon_1$ \\ \hline 
%			$\astar < \bstar$ & $\epsilon_1\epsilon_2 < 1$ \\ \hline 
			$\bstar < 1$ & $d_1 < \epsilon_1$ \\
			\hline
		\end{tabular}
	\end{center}
	\caption{We justify the ordering of the region boundaries of Figure~\ref{fig:regions_d1_mid} when $2(\epsilon_1\epsilon_2 - 1)/\epsilon_2 < d_1 < \epsilon_1^2\epsilon_2$.  In the left column, we have the ordering between two boundary points, and in the right column, we show the necessary and sufficient condition that justifies the ordering.}	
	\label{tab:d1_mid}	
\end{table}


==> one_sided/fig/indep/d1_small_fig_tab_indep.tex <==
% -------------------------------------------------------------
% d_1 < 
% -------------------------------------------------------------

\begin{figure}
	\centering
%	\includegraphics[scale=0.8]{3/one_sided/fig/system_model_one_sided}
	\includegraphics[scale=1]{3/one_sided/fig/regions_d1_small}
%%	\includegraphics[width=0.6\textwidth]{outer_bound.png}
	\caption{The different regions requiring separate coding schemes when $0 \leq d_1 \leq 2(\epsilon_1\epsilon_2 - 1)/\epsilon_2$.}
	\label{fig:regions_d1_small}
\end{figure}

\begin{table}
	\begin{center}
		\begin{tabular}{| c | c |}
%    \caption{The justification for the ordering}
			\hline
			\multicolumn{2}{|c|}{{\bf Ordering of Boundaries for $\depstwo$ when $0 \leq d_1 \leq 2(\epsilon_1\epsilon_2 - 1)/\epsilon_2$}} \\
			\hline
			{\bf Inequality} & {\bf Justification}   \\ \hline
			$d_1 < d_1/\epsilon_1$ & $\epsilon_1 < 1$ \\ \hline 
			$d_1/\epsilon_1 < d_1 + (1 - \epsilon_1)$ & $d_1 < 1$ \\ \hline 
			$d_1 + (1 - \epsilon_1) \leq \astar$ & $d_1 \leq 2(\epsilon_1\epsilon_2 - 1)/\epsilon_2$ \\ \hline 
			$\astar < \bstar$ & $\epsilon_1\epsilon_2 < 1$ \\ \hline 
			$\bstar < 1$ & $d_1 < \epsilon_1$ \\
			\hline
		\end{tabular}
	\end{center}
	\caption{We justify the ordering of the region boundaries of Figure~\ref{fig:regions_d1_small} when $0 \leq d_1 \leq 2(\epsilon_1\epsilon_2 - 1)/\epsilon_2$.  In the left column, we have the ordering between two boundary points, and in the right column, we show the necessary and sufficient condition that justifies the ordering.}	
	\label{tab:d1_small}
\end{table}

==> one_sided/independent/one_sided_optimality_indep.tex <==
\subsection{Minmax Latency Optimality}
\label{sec:one_sided_optimality}

In this section, we show that it is possible to choose values for $\omegaparam, \gammaparam \in [0, 1]$ from Section~\ref{subsubsec:inner_bound} so that the lower bound for the minmax latency in~\eqref{eq:wplusd} is achieved.  We first calculate the expected number of \emph{unknown} variables involved in transmissions to the weaker user from Phase~\Rmnum{2} onwards.  

First, since we send random linear combinations of the symbols in $\Fset$ in Phase~\Rmnum{2}, we initially expect this to contribute $|\Fset|$ variables.  However, the probability that any symbol in $\Fset$ was not already received by the weaker user in Phase~\Rmnum{1} is equal to $\epsilon_2$.  Therefore the expected number of \emph{unknown} variables within $\Fset$ is given by $\nFUnknown$, where

\setcounter{cnt}{1}
\begin{align}
	\mathbb{E}\nFUnknown &= \mathbb{E}|\Fset|\epsilon_2 \\
	&= \mathbb{E}|\BsetOmega \cup \Cset|\epsilon_2 \\
	&\stackrel{(\alph{cnt})}{=} \left( \mathbb{E}|\BsetOmega| + \mathbb{E} |\Cset| \right) \epsilon_2	 \\
	\addtocounter{cnt}{1}
	\label{eq:nFUnknown}	
	&\stackrel{(\alph{cnt})}{=}  N\left( \omegaparam(\epsilon_1 - d_1) + \gamma(1 - \epsilon_1) \right)\epsilon_2
\end{align}
where 
\begin{enumerate}[(a)]
	\item follows from the fact that $\BsetOmegaC$ and $\Cset$ are disjoint by construction
	\item follows by construction (see Section~\ref{subsubsec:inner_bound} and Figure~\ref{fig:set_construction}).
\end{enumerate}

The use of repetition coding for the symbols in $\BsetOmegaC$ in Phase~\Rmnum{2} further adds additional unknown variables to the coding scheme.  On average, the expected number of symbols repeated is $\mathbb{E}|\BsetOmegaC| = N(1  - \omegaparam)(\epsilon_1 - d_1)$, of which, again, only an $\epsilon_2$ fraction were not already received by the weaker user in Phase~\Rmnum{1}.  By Lemma~\ref{lem:repetition}, the number of additional \emph{unknown} variables introduced to the weaker user as a result of the repetition scheme is therefore given by $\nBUnknown$, where

\setcounter{cnt}{1}
\begin{align}
	\label{eq:nBUnknown}
	\mathbb{E}\nBUnknown &= N(1  - \omegaparam)(\epsilon_1 - d_1)\epsilon_2 \frac{1 - \epsilon_2}{1 - \epsilon_1\epsilon_2}.
\end{align}

Let $\LHSfuncparam$ be the expected fraction of all source symbols that are involved in transmissions to the weaker user from Phase~\Rmnum{2} onwards that have not yet been decoded prior to Phase~\Rmnum{2}.  We have that $\LHSfuncparam$ is the normalized sum of~\eqref{eq:nFUnknown} and~\eqref{eq:nBUnknown}, i.e., 

\begin{align}
	\LHSfuncparam &= \frac{\mathbb{E}\nFUnknown + \mathbb{E}\nBUnknown}{N} \\
	&= \kgamma \gammaparam + \komega \omegaparam	+ \kk
	\label{eq:LHSfuncparam}
\end{align}
where 
\begin{subequations}
\begin{align}
	\kgamma &= (1 - \epsilon_1)\epsilon_2, \label{eq:kgamma} \\	
	\komega &= \frac{\epsilon_{2}^{2}(\epsilon_1 - d_1)(1 - \epsilon_1)}{1 - \epsilon_1\epsilon_2}, 	\label{eq:komega}\\
	\kk &= \frac{\epsilon_{2}(\epsilon_1 - d_1)(1 - \epsilon_2)}{1 - \epsilon_1\epsilon_2}.
	\label{eq:kk}
\end{align}
\end{subequations}

Having calculated the number of unknown variables sent to the weaker user from Phase~\Rmnum{2} onwards, we now consider the number of equations he receives in Phases~\Rmnum{2} and~\Rmnum{3}.  From Section~\ref{subsubsec:inner_bound}, we know that during these phases, the total number of transmissions was simply equal to the number of trials needed to send $N(\epsilon_1 - d_1)$ equations to the stronger user with feedback.  The number of transmissions in Phases~\Rmnum{2} through~\Rmnum{3}  is therefore distributed according to a negative binomial distribution and the mean number of transmissions in this period is $W_{2,3} = N(\epsilon_1 - d_1)/(1 -\epsilon_1)$.  Of these transmissions, the expected number received by the weaker user is equal to $W_{2, 3}(1 - \epsilon_2)$.  We therefore define the capacity of the weaker user's channel during Phases~\Rmnum{2} through~\Rmnum{3} as $C_{2,3}$, where

\begin{align}
	C_{2,3} = \frac{(\epsilon_1 - d_1)(1 - \epsilon_2)}{1 - \epsilon_1},
%	\bstar &= \frac{(1 - \epsilon_1) + d_1(1 - \epsilon_2)}{1 - \epsilon_1\epsilon_2}
\end{align}
%and the expected number of equations received by the weaker user in Phases~\Rmnum{2} through~\Rmnum{3} is given by $NC_{2, 3}$.  
We next compare $\LHSfuncparam$, the amount of source symbols destined for the weaker user, with $NC_{2, 3}$,  the capacity supported over the weaker user's channel during Phases~\Rmnum{2} and~\Rmnum{3}.  

As mentioned in Section~\ref{subsubsec:inner_bound}, the weaker user requires an additional $N(\epsilon_2 - d_2)$ symbols to be sent from Phase~\Rmnum{2} onwards.  Therefore, it is necessary that $\LHSfuncparam \geq \epsilon_2 - d_2$.  However, if $\LHSfuncparam$ is much greater than $\epsilon_2 - d_2$, we encounter the problem explained in the introduction of this section in which the weaker user is forced to decode unnecessary symbols thus introducing delay.  Say that we are able to find values of $\gammaparam', \omegaparam' \in [0, 1]$ such that $\LHSfuncprime = \epsilon_2 - d_2$.  We consider two cases when this is so -- when $\LHSfuncprime \leq C_{2, 3}$ and when $\LHSfuncprime > C_{2, 3}$.  We show that in both cases, we can achieve the optimal minmax  latency so long as $\LHSfuncprime = \epsilon_2 - d_2$.

In the first case, when $\LHSfuncprime \leq C_{2, 3}$, we wish to send less information over the channel than what the channel capacity can support.  Therefore, we expect that the weaker user should be able to decode all source symbols before the conclusion of Phase~\Rmnum{3}.  However, in general, if the weaker user achieves distortion $d_2$ after decoding, it will be at a latency $w$, where $w > \wtwo$.  That is, in general, the weaker user may not achieve an \emph{individual} point-to-point optimal latency.

To see why this is so, recall from Section~\ref{subsubsec:inner_bound} that in Phase~\Rmnum{2} of our coding scheme, we transmit $\bOmegaT + v(t)$ at every time instant $t$, where $v(t)$ is a new random linear combination of the source symbols in $\Fset$ generated at every time $t$.  Since $\LHSfuncprime \leq C_{2, 3}$, there is the possibility that at some point, the weaker user is able to decode all symbols in $\Fset$ even before Phase~\Rmnum{2} has concluded.  Say that this is the case and the stronger user has stalled on receiving a particular symbol $\bOmegaC \in \BsetOmegaC$ being repeated.  Let us further assume that the weaker user has already received $\bOmegaC$.  Then while $\bOmegaC + v(t)$ is being transmitted, all transmissions to the weaker user are redundant.
%and thus the reception of a channel symbol will not lead to the acquisition of an independent equation that can be used to decode an additional source symbol.  
After $\bOmegaC$ is received by the stronger user and the transmitter moves on to  $\bOmegaPrime$, the next symbol in $\BsetOmegaC$ to be sent via the modified repetition scheme, the weaker user can continue to receive innovative information.  However, the set of transmissions received while $\bOmegaC$ is being repeated prevents the weaker user from achieving an optimal \emph{individual} latency.

However, we show that the optimal \emph{minmax} latency can still be achieved.  Notice that the moment all symbols in $\Fset$ can be decoded by the weaker user, the random linear combination $v(t)$ can be subtracted from any transmission $\bOmegaT + v(t)$ in Phase~\Rmnum{2}.  Therefore the remainder of Phase~\Rmnum{2} effectively consists of uncoded transmissions from the weaker user's perspective, and he is eventually able to decode all $\LHSfuncprime$ symbols.  Thus, so long as $\LHSfuncprime = \epsilon_2 - d_2$, the weaker user will decode the necessary amount of symbols before the conclusion of Phase~\Rmnum{3}, while the stronger user decodes at an optimal latency the moment Phase~\Rmnum{3} terminates.  In this case, the stronger user is the bottleneck of the system and in fact, the condition $\LHSfuncprime \leq C_{2, 3}$ is equivalent to $w_{1}(d_1) \geq w_2(d_2)$.  

%For example, say that $\bOmegaPrime$ is the last symbol in $\BsetOmegaC$ about to be sent via the modified repetition coding at time $t_2$.  

%Although the weaker user receives $NC_{2, 3}$ equations during Phases~\Rmnum{2} through~\Rmnum{3}, it may not necessarily be the case that all equations are independent.  Recall from Section~\ref{subsubsec:inner_bound} that in Phase~\Rmnum{2} of our coding scheme, we transmit $\bOmegaT + v(t)$ at every time instant $t$, where $v(t)$ is a new random linear combination of the source symbols in $\Fset$ generated at every time $t$.  There is the possibility that at some point, the weaker user is able to decode all symbols in $\Fset$ even before Phase~\Rmnum{2} has concluded.  

%Notice however, that the moment the weaker user can decode all source symbols in $\Fset$, the only remaining symbols missing are those in $\BsetOmegaC$.  Therefore, during Phase~\Rmnum{2} when $\bOmegaT + v(t)$ is being repeated, the weaker user can subtract off $v(t)$, and can thereby 

%may not necessarily lead to an \emph{independent} equation received.  

%Now, although the weaker user receives $NC_{2, 3}$ equations during Phases~\Rmnum{2} through~\Rmnum{3}, it may not necessarily be the case that all equations are independent.  Recall from Section~\ref{subsubsec:inner_bound} that in Phase~\Rmnum{2} of our coding scheme, we transmit $\bOmegaT + v(t)$ at every time instant $t$, where $v(t)$ is a new random linear combination of source symbols in $\Fset$ generated at every time $t$.  There is the possibility that at some point, the weaker user is able to decode all symbols in $\Fset$ even before Phase~\Rmnum{2} has concluded.  If this is the case and the stronger user has stalled on receiving a particular symbol being repeated that the weaker user has already received, then all transmissions to the weaker user will be redundant, and thus the reception of a channel symbol will not lead to the acquisition of an independent equation that can be used to decode an additional source symbol.  

%we will have received more equations than unknown variables and so the weaker user can decode at the conclusion of Phase~\Rmnum{3}.  In this case, the stronger user is the bottleneck of the system and the condition $\LHSfuncprime \leq C_{2, 3}$ is equivalent to $w_{1}(d_1) \geq w_2(d_2)$.  

On the other hand, if $\LHSfuncprime > C_{2, 3}$, the weaker user has more unknown variables than equations and so he cannot yet decode at the conclusion of Phase~\Rmnum{3}.  However, every transmission he has received so far is ``innovative'' in the sense that it provides an independent equation that can be used to decode the $N\LHSfuncprime$ source symbols.  In order to decode, we simply need to send more equations to the weaker user, and since $\LHSfuncprime = \epsilon_2 - d_2$, there will not be any unnecessary source symbols sent.  Since the stronger user is point-to-point optimal at the conclusion of Phase~\Rmnum{3}, we have therefore sent a total of $Nw_1(d_1)$ transmissions up to that point.  Since, from the weaker user's perspective, we have hitherto been sending random linear combinations of $N\LHSfuncprime$ variables, we simply need to continue doing so for another $N(w_2(d_2) - w_1(d_1))$ transmissions in Phase~\Rmnum{4} before he receives the remaining number of equations required and achieves point-to-point optimal performance.

\begin{table}
	\begin{center}
		\begin{tabular}{| c | c |}
%    \caption{The justification for the ordering}
			\hline
			\multicolumn{2}{|c|}{{\bf Ordering of Boundaries for $d_1$}} \\
			\hline
			{\bf Inequality} & {\bf Justification}   \\ \hline
			$2(\epsilon_1\epsilon_2 - 1)/\epsilon_2 < \epsilon_1^2\epsilon_2$ & $(1 - \epsilon_1\epsilon_2)^2 > 0$ \\ \hline 
			$\epsilon_1^2\epsilon_2 < \epsilon_1$ & $\epsilon_1\epsilon_2 < 1$, $\epsilon_1 > 0$ \\ \hline 
			\hline
		\end{tabular}
	\end{center}
	\caption{We justify the ordering of the region boundaries for $d_1$.  In the left column, we have the ordering between two boundary points, and in the right column, we show the necessary and sufficient condition that justifies the ordering.}	
	\label{tab:d1_boundaries}	
\end{table}


We therefore see that regardless of whether $\LHSfuncparam$ is greater or less than $C_{2, 3}$, we can achieve an optimal minmax latency so long as we can find $\gammaparam, \omegaparam \in [0, 1]$ such that $\LHSfuncparam = \epsilon_2 - d_2$.   We focus on finding these values of $\gammaparam$ and $\omegaparam$ in the next sections. In doing so, we consider three cases cases for $d_1$.  The first is when $0 \leq d_1 \leq 2(\epsilon_1\epsilon_2 - 1)/\epsilon_2$, the second when $2(\epsilon_1\epsilon_2 - 1)/\epsilon_2 < d_1 < \epsilon_1^2\epsilon_2$, and third when $\epsilon_1^2\epsilon_2 \leq d_1 < \epsilon_1$.  We justify the position of these boundary points with Table~\ref{tab:d1_boundaries}.  For example, in the first row of Table~\ref{tab:d1_boundaries}, we justify that the boundary point $2(\epsilon_1\epsilon_2 - 1)/\epsilon_2$ is less than the boundary point $\epsilon_1^2\epsilon_2$ with the necessary and sufficient condition that $(1 - \epsilon_1\epsilon_2)^2 > 0$.  

After dividing the values of $d_1$ into regions, we then further consider regions of $d_2/\epsilon_2$, where each region requires a distinct choice for the values of $\gammaparam$ and $\omegaparam$.  Recall from Remark~\ref{rem:deps} in Section~\ref{sec:system_model} that for $i \in \{1, 2\}$, we assume that $d_i/\epsilon_i < 1$, otherwise the coding is trivial.  Therefore, we consider only values of $d_2/\epsilon_2 \in [0, 1]$.  In the following sections, the regions of $\depstwo$ will depend on the boundaries $\astar$ and $\bstar$, which we define as

%Within each case that $d_1$ falls into, we further consider regions for $d_2$ that require separate choices of $\gammaparam$ and $\omegaparam$ so that $\LHSfuncparam = \epsilon_2 - d_2$.  These regions depend on the boundaries $\astar$ and $\bstar$, which we define as

\begin{align}
	\astar &= \frac{\epsilon_1\epsilon_2(1 - \epsilon_1) + d_1(1 - \epsilon_2)}{1 - \epsilon_1\epsilon_2}, \\
	\bstar &= \frac{(1 - \epsilon_1) + d_1(1 - \epsilon_2)}{1 - \epsilon_1\epsilon_2}.
\end{align}

\input{3/one_sided/optimality_regions}

==> one_sided/independent/optimality_regions_indep.tex <==
\subsubsection{Case~\Rmnum{1}: $0 \leq d_1 \leq 2(\epsilon_1\epsilon_2 - 1)/\epsilon_2$}

\input{3/one_sided/fig/d1_small_fig_tab}

We first mention that the upper bound in the assumption $d_1 \leq 2(\epsilon_1\epsilon_2 - 1)/\epsilon_2$ can be either positive or negative depending on the values of $\epsilon_1$ and $\epsilon_2$.  In the case that the upper bound is positive and $d_1$ is in this region, we now go through the process of finding the values of $\gammaparam$ and $\omegaparam$ such that $\LHSfuncparam = \epsilon_2 - d_2$.  

%We will see that this region is the most difficult in the sense that it has the most distinct coding regions and 

We begin by dividing the number line for $\depstwo$ in Figure~\ref{fig:regions_d1_small}, where we have justified the ordering of each boundary point with Table~\ref{tab:d1_small}.  For example, in the third row of the table, we justify the ordering that $d_1 + (1 - \epsilon_1) \leq \astar$ with the necessary and sufficient condition that $d_1 \leq 2(\epsilon_1\epsilon_2 - 1)/\epsilon_2$, which is the assumption in this region of $d_1$ that we consider.  We enumerate all regions of Figure~\ref{fig:regions_d1_small} and provide the values of $\gammaparam$ and $\omegaparam$.

%\renewcommand{\labelenumi}{[\theenumi]} 
%\begin{description}[before={\renewcommand\makelabel[1]{\bfseries ##1.}}]
%    \setcounter{enumi}{#1}
%    \addtocounter{enumi}{1}

\begin{description}
	\item[Region~\Rmnum{5}] In this region, we set $\gammaparam = \omegaparam = 0$ and recover the unmodified repetition coding scheme discussed in the beginning of Section~\ref{subsubsec:repetition_coding}.  In fact, we do not require that $\LHSfuncparam = \epsilon_2 - d_2$ in this region.  Instead, by sending all $N(\epsilon_1 - d_1)$ source symbols uncoded, by Lemma~\ref{lem:repetition}, we can work out that $N\kk$ uncoded source symbols are received by the weaker user, where $\kk$ is given by~\eqref{eq:kk}.  We can confirm that in Region~\Rmnum{5}, in which $\depstwo \geq \bstar$, the distortion requirement of the weaker user is sufficiently large so that it can be met by the amount of uncoded symbols he receives.
	\item[Region~\Rmnum{4}] In this region, we set $\omegaparam = 0$, and $\gammaparam = \gammatilde$ where 
		\begin{align}
			\gammatilde &= \frac{(\epsilon_2 - d_2)(1 - \epsilon_1\epsilon_2) - \epsilon_2(\epsilon_1 - d_1)(1 - \epsilon_2)}{(1 - \epsilon_1)\epsilon_2}.
			\label{eq:gammatilde}
		\end{align}
		Within this region, the weaker user's distortion constraint is sufficiently low so that additional coded symbols must be transmitted.  We can confirm that this choice of $\gammaparam$ and $\omegaparam$ results in $\LHSfuncparam = \epsilon_2 - d_2$ in~\eqref{eq:LHSfuncparam}.  Furthermore, the conditions $\gammatilde \geq 0$ and $\gammatilde \leq 1$ are equivalent to $\depstwo \leq \bstar$ and $\depstwo \geq \astar$ respectively, which are satisfied in this region.
	\item [Region~\Rmnum{3}]  In this region, we set $\gammaparam = 0$ and $\omegaparam = \omegastar$, where
		\begin{align}
			\omegastar &= \frac{(\epsilon_2 - d_2)(1 - \epsilon_1\epsilon_2) - \epsilon_2(\epsilon_1 - d_1)(1 - \epsilon_2)}{\epsilon_{2}^{2}(\epsilon_1 - d_1)(1 - \epsilon_1)}.
		\end{align}
		We can confirm that this choice of $\gammaparam$ and $\omegaparam$ results in $\LHSfuncparam = \epsilon_2 - d_2$ in~\eqref{eq:LHSfuncparam}.  Furthermore, the conditions $\omegastar \geq 0$ and $\omegastar \leq 1$ are equivalent to $\depstwo \leq \bstar$ and $\depstwo \geq d_1 + (1 - \epsilon_1)$ respectively, which are satisfied in this region.%		To see how we derive this value of $\omegaparam$, we first consider~\eqref{eq:LHSfuncparam}.
	
	\item[Region~\Rmnum{2}]  In this region, we set $\omegaparam= 1$, $\gammaparam = \gammahat$, where
		\begin{align}
			\gammahat &= \frac{(\epsilon_2 - d_2) - (\epsilon_1 - d_1)\epsilon_2}{(1 - \epsilon_1)\epsilon_2}.
			\label{eq:gammahat}
		\end{align}
		We can confirm that this choice of $\gammaparam$ and $\omegaparam$ results in $\LHSfuncparam = \epsilon_2 - d_2$ in~\eqref{eq:LHSfuncparam}.  Furthermore, the conditions $\gammahat \geq 0$ and $\gammahat \leq 1$ are equivalent to $\depstwo \leq d_1 + (1 - \epsilon_1)$ and $\depstwo \geq d_1$ respectively, which are satisfied in this region.%		To see how we derive this 
	
	\item[Region~\Rmnum{1}]  In this region, we ignore feedback altogether and use the successive segmentation coding scheme of the previous chapter, which showed in Section~\ref{subsubsec:two_users} that both users can be point-to-point optimal if $\depstwo \leq \depsone$.
\end{description}

%\begin{enumerate}[label = \uline{\textit{Step \arabic*:}}]
%	\item hello
%\end{enumerate}
%\begin{etaremune}[label = \uline{\textit{Step \arabic*:}}]
%\end{etaremune}
%\begin{description}
%	\item[ Region~\Rmnum{5}: $\gammaparam = \omegaparam = 0$]  In this region 
%\end{description}


\subsubsection{Case~\Rmnum{2}: $2(\epsilon_1\epsilon_2 - 1)/\epsilon_2 < d_1 < \epsilon_1^2\epsilon_2$}

We again divide the number line for $\depstwo$ in Figure~\ref{fig:regions_d1_mid} where we have justified the ordering of each boundary point with Table~\ref{tab:d1_mid}.  Notice however, that in the ranges of $d_1$ we now consider, the boundary points $\astar$ and $d_1 + (1 - \epsilon_1)$ have swapped positions compared to Figure~\ref{fig:regions_d1_small}.  We again enumerate all regions of Figure~\ref{fig:regions_d1_mid}.

\input{3/one_sided/fig/d1_mid_fig_tab}

\begin{description}
	\item[Region~\Rmnum{9}] In this region, we set $\gammaparam = \omegaparam = 0$ and recover the unmodified repetition coding scheme discussed in the beginning of Section~\ref{subsubsec:repetition_coding} (see the description of Region~\Rmnum{5} in the previous section).

	\item[Region~\Rmnum{8}] In this region, we set $\omegaparam = 0$, and $\gammaparam = \gammatilde$ where $\gammatilde$ is given by~\eqref{eq:gammatilde} (see the description of Region~\Rmnum{4} in the previous section).
	
	\item[Region~\Rmnum{7}]  In this region, we set $\omegaparam= 1$, $\gammaparam = \gammahat$, where $\gammahat$ is given by~\eqref{eq:gammahat} (see the description of Region~\Rmnum{2} in the previous section).

	
	\item[Region~\Rmnum{6}]  In this region, we again ignore feedback altogether and use the successive segmentation coding scheme of the previous chapter (see the description of Region~\Rmnum{1} in the previous section).
\end{description}

\subsubsection{Case~\Rmnum{3}: $\epsilon_1^2\epsilon_2 \leq d_1 < \epsilon_1$}

For the final case of $d_1$ we consider, we again divide the number line for $\depstwo$ in Figure~\ref{fig:regions_d1_big}, where we have justified the ordering of each boundary point with Table~\ref{tab:d1_big}.  Again, the values of $d_1$ we consider have resulted in some of the boundaries in Figure~\ref{fig:regions_d1_big} moving relative to Figure~\ref{fig:regions_d1_mid}, most notably that now $\astar < \depsone$.  We again enumerate all regions of Figure~\ref{fig:regions_d1_mid}.

\input{3/one_sided/fig/d1_big_fig_tab}

\begin{description}
	\item[Region~\Rmnum{12}] In this region, we set $\gammaparam = \omegaparam = 0$ and recover the unmodified repetition coding scheme discussed in the beginning of Section~\ref{subsubsec:repetition_coding} (see the description of Region~\Rmnum{5} in the previous section).

	\item[Region~\Rmnum{11}] In this region, we set $\omegaparam = 0$, and $\gammaparam = \gammatilde$ where $\gammatilde$ is given by~\eqref{eq:gammatilde} (see the description of Region~\Rmnum{4} in the previous section).

	
	\item[Region~\Rmnum{10}]  In this region, we again ignore feedback altogether and use the successive segmentation coding scheme of the previous chapter (see the description of Region~\Rmnum{1} in the previous section).
\end{description}



==> one_sided/independent/repetition_coding_indep.tex <==
\subsubsection{Repetition Coding}
\label{subsubsec:repetition_coding}

Consider a coding scheme that simply ignores the weaker user and focuses on using the stronger user's feedback to retransmit each of his required source symbols until it is received.  We wish to calculate the expected value of $\Nretransmit$, which we define as the number of \emph{unique} source symbols received by the weaker user when $k \in \mathbb{N}$ symbols are to be sent to the stronger user via repetition coding.

Let $\nRepi{i}$ be a random variable representing the number of transmissions needed to be sent for symbol $S(i)$ to be received by the \emph{stronger} user, user~1, in the repetition scheme.  Let $\indi{i}$ be an indicator variable indicating whether symbol $S(i)$ was received by the \emph{weaker} user, user~2, in any of the $\nRepi{i}$ transmissions and let $\vecnRep = \{\nRepi{1}, \nRepi{2}, \ldots, \nRepi{k}\}$ be the vector of random variables giving the number of repetitions needed to send each source symbol.  %Lastly, let $\Nretransmit$ be the number of unique source symbols received by the weaker user during the repetition scheme for the stronger user.  
Given $\vecnRep$, we calculate $\mathbb{E}(\Nretransmit | \vecnRep)$ as 

\setcounter{cnt}{1}
\begin{align}
	\mathbb{E}(\Nretransmit | \vecnRep) &= \sum_{i = 1}^{k} \mathbb{E}(\indi{i} | \vecnRep) \\
	&= \sum_{i = 1}^{k} \Prob(\text{user~2 receives } S(i) | \vecnRep) \\
%	\addtocounter{cnt}{1}
	&\stackrel{(\alph{cnt})}{=} \sum_{i = 1}^{k} \left\{1 - \textrm{Pr}(Z_2(t) = 1 | Z_{1}(t) = 1)^{\nRepi{i} - 1}\textrm{Pr}(Z_2(t) = 1 | Z_{1}(t) = 0) \right\}\\
	\addtocounter{cnt}{1}	
	\label{eq:Nretransmit_g_Mi}	
	&\stackrel{(\alph{cnt})}{=} \sum_{i = 1}^{k} \left\{1 - \left( \frac{\epsot}{\epsilon_1} \right)^{\nRepi{i} - 1} \left(\frac{\epsilon_2 - \epsot}{1 - \epsilon_1}\right)\right\}
%	\addtocounter{cnt}{1}	
%	&\stackrel{(\alph{cnt})}{=}  k - \sum_{i = 0}^{k} \epsilon_{2}^{\nRepi{i}} \\
\end{align}
where 
\begin{enumerate}[(a)]
	\item follows by construction of the repetition-based scheme
	\item we have calculated the conditional probabilities from~\eqref{eq:pmf_z1z2}.
\end{enumerate}

\setcounter{cnt}{1}
We next use the law of total probability to get that 
\begin{align}
	\ENretransmit &= \sum_{\vecnRep} \mathbb{E}(\Nretransmit | \vecnRep) \Prob(\vecnRep) \\
	&\stackrel{(\alph{cnt})}{=} \sum_{\vecnRep} \sum_{i = 1}^{k} \left\{1 - \left( \frac{\epsot}{\epsilon_1} \right)^{\nRepi{i} - 1} \left(\frac{\epsilon_2 - \epsot}{1 - \epsilon_1}\right)\right\}  \Prob(\vecnRep) \\
	\addtocounter{cnt}{1}
	&\stackrel{(\alph{cnt})}{=} \sum_{i = 1}^{k}  \sum_{j= 1}^{\infty}  \left\{1 - \left( \frac{\epsot}{\epsilon_1} \right)^{\nRepi{i} - 1} \left(\frac{\epsilon_2 - \epsot}{1 - \epsilon_1}\right)\right\} \Prob(\nRepi{i} = j)  \\
	\addtocounter{cnt}{1}
	&= k - \left(\frac{\epsilon_2 - \epsot}{1 - \epsilon_1}\right)\sum_{i = 1}^{k}  \sum_{j= 1}^{\infty} \epsilon_{2}^{j} \Prob(\nRepi{i} = j)  \\
	&\stackrel{(\alph{cnt})}{=} k - \sum_{i = 1}^{k}  \sum_{j= 1}^{\infty} \epsilon_{2}^{j} (\epsilon_{1}^{j - 1}(1 - \epsilon_1))  \\
	\addtocounter{cnt}{1}	
	&= k \left( 1 - \epsilon_2(1 - \epsilon_1)  \sum_{j= 1}^{\infty} (\epsilon_{1}\epsilon_2)^{j-1}   \right) \\
%	\addtocounter{cnt}{1}	
	&\stackrel{(\alph{cnt})}{=} k \left( 1 - \epsilon_2(1 - \epsilon_1) \left\{ \frac{1}{1 - \epsilon_1\epsilon_2}\right\}   \right) \\
	\label{eq:ENretransmit}
	&=  k \cdot \frac{1 - \epsilon_2}{1 -\epsilon_1\epsilon_2}
\end{align}
where 
\begin{enumerate}[(a)]
	\item follows from~\eqref{eq:Nretransmit_g_Mi}
	\item follows from the fact that the $\nRepi{i}$ are i.i.d.
	\item follows from the fact that by construction, $\nRepi{i}$ is a geometric random variable with probability of success $(1 - \epsilon_1)$
	\item follows from the formula for the geometric series and the fact that $\epsilon_1\epsilon_2 < 1$.
\end{enumerate}

\begin{myLemma}
\label{lem:repetition}
	Let $k$ source symbols be sent to the stronger user via a repetition scheme.  Then $\ENretransmit $, the expected number of unique source symbols received by the weaker user, is given by~\eqref{eq:ENretransmit}.
\end{myLemma}

==> one_sided/one_sided_inner_bound_backup.tex <==
\subsubsection{Inner Bound}
\label{subsubsec:inner_bound}

In this section, we formulate a hybrid coding scheme that incorporates both repetition coding and sending random linear combinations of source symbols.  The code is tuned via two parameters, $\omegaparam, \gammaparam \in [0, 1]$.  We target the point-to-point optimal distortion/latency for the stronger user in this section, and show that the stronger user can achieve point-to-point optimal performance for any values of $\omegaparam$ and $\gammaparam$.  In the next section however, we show how to optimize $\omegaparam$ and $\gammaparam$ to also achieve point-to-point optimal performance for the weaker user.  As in the coding scheme in Section~\ref{sec:two_users}, we again split the coding scheme into phases.  

In Phase~\Rmnum{1}, we begin by sending each source symbol uncoded over the channel.  That is, Phase~\Rmnum{1} consists of $N$ transmissions and at time $t \in \{1, 2, \ldots, N\}$, we transmit $X(t) = S(t)$.  Let $\Aset \subseteq [N]$ be the set of symbols received by the stronger user in Phase~\Rmnum{1}.  Since the stronger user's feedback is available to all receivers and the transmitter, $\Aset$ is known to all parties.  
%We have that $\mathbb{E}|A| = 1 - \epsilon_1$ 

At the conclusion of Phase~\Rmnum{1}, we have that on average, for $i \in \{1, 2\}$, user~$i$ will have received $N(1 - \epsilon_i)$ source symbols and so will require an additional $N(\epsilon_i - d_i)$ symbols in the remaining phases.   Before moving on to Phase~\Rmnum{2}, we first organize the source symbols in $\Aset$ and $\AsetC$ into subsets, where $\AsetC \subseteq [N]$ denotes the complement of set $\Aset$. We first isolate a fraction of $N(\epsilon_1 - d_1)$ source symbols from $\AsetC$ into a set denoted as $\Bset$.  That is, we fix the remaining $N(\epsilon_1 - d_1)$ symbols that the stronger user requires in $\Bset$.  We then partition $\Bset$ into two disjoint sets, one that contains a fraction of $\omegaparam \in [0, 1]$ source symbols from $\Bset$, denoted as $\BsetOmega$, and the other that contains a fraction of $1 - \omegaparam$ symbols, denoted as $\BsetOmegaC$, where $\Bset = \BsetOmega \cup \BsetOmegaC$.  Random linear combinations of the symbols in $\BsetOmega$ will be sent to the stronger user while the symbols in $\BsetOmegaC$ will be sent with repetition coding.  We further take a fraction of $\gammaparam \in [0, 1]$ source symbols from $\Aset$ and denote this set as $\Cset$.  Finally, we define $\Fset$ as the union of sets $\Cset$ and $\BsetOmega$.  Figure~\ref{fig:} illustrates the relationship between all sets and the manner in which they are constructed.

In Phase~\Rmnum{2} of the coding scheme, we send random linear combinations of the source symbols in $\Fset \triangleq \Cset \cup \BsetOmega$.  Let $v(t)$ be a \emph{new} random linear combination of the source symbols in $\Fset$ generated at time $t$.  Since $\Cset \subseteq \Aset$, the stronger user can subtract off all symbols originating from $\Cset$ and so the only symbols providing new information are those originating from $\BsetOmega$.  We use the stronger user's feedback to continue to send random linear combinations until the stronger user has received $|\BsetOmega|$ equations, where $\mathbb{E}|\BsetOmega| = \omegaparam(\epsilon_1 - d_1)$.  At the conclusion of Phase~\Rmnum{2}, by construction, the stronger user has decoded all symbols in $\Fset$.

In Phase~\Rmnum{3}, we use a repetition coding scheme to send each symbol $\bOmegaC \in \BsetOmegaC$.  However, since all symbols in $\Fset$ have been decoded by the stronger user at the beginning of Phase~\Rmnum{3}, notice that we can also combine the symbol $\bOmegaC$ with a random linear combination of the symbols in $\Fset$ to the benefit of the weaker user, but at no extra cost to the stronger user.  That is, let $\bOmegaC$ be a symbol that would be sent with a repetition scheme at time $t$.  Then instead of transmitting $\bOmegaC$ at time $t$, we instead transmit $v'(t) = v(t) + \bOmegaC$ where $v(t)$ is a \emph{new} random linear combination of the source symbols in $\Fset$, which can be subtracted off by the stronger user.
As with a conventional repetition scheme, we also repeat $\bOmegaC$ until it is received by the stronger user for all $\bOmegaC \in \BsetOmegaC$.  However, the difference in Phase~\Rmnum{3} is that we also combine $\bOmegaC$ with $v(t)$, a different linear combination of the source symbols in $\Fset$ at every retransmission.  At the conclusion of Phase~\Rmnum{3} it is not hard to see that the stronger user achieves point-to-point optimal performance, since every channel symbol received has lead to the decoding of a source symbol.  

Finally, in Phase~\Rmnum{4}, if the weaker user has not yet met his distortion constraint, we continue to send random linear combinations of the source symbols in $\Fset$.

%instead of sending the random linear combination $v(t)$ at time $t$ as in Phase~\Rmnum{2}, we instead transmit $v'(t) = v(t) + \bOmegaC$ where $\bOmegaC \in \BsetOmegaC$ is a source symbol that has yet to be received by the stronger user.  Since the stronger user has decoded all symbols in $\Fset$ from the previous phase, he can subtract off $v(t)$ from $v'(t)$ at any time $t$ in Phase~\Rmnum{3}. 



==> one_sided/problem_formulation_bak.tex <==
\subsection{Problem Formulation}
\label{sec:system_model_one_sided}

%\subsection{{}System Model}
%\section{Problem Formulation}

%We first define the problem in Section~\ref{subsec:problem_definition}.  In Section~\ref{subsec:metrics}, we then discuss metrics that are of interest in the evaluation of broadcast codes and show how a solution to the problem in Section~\ref{subsec:problem_definition} can be used to address these metrics.

%\input{2_problem_formulation/problem_definition}
%\input{2_problem_formulation/metrics}

%%%\begin{figure*}
%%\begin{figure}
%%	\centering
%%%	\input{3/out/fig/schematic}
%%%	\includegraphics[scale=0.6]{3/out/fig/schematica}
%%%	\includegraphics[scale=0.75]{out/fig/schematic}
%%%	\includegraphics[scale=0.8]{2_problem_formulation/fig/schematicE}
%%	\includegraphics{2_problem_formulation/fig/schematicE}
%%%	\includegraphics[width=0.6\textwidth]{outer_bound.png}
%%	\caption{Broadcasting an equiprobable binary source over an erasure broadcast channel.}
%%	\label{fig:schematic}
%%%\end{figure*}
%%\end{figure}

%We begin by presenting our joint source-channel coding formulation which is illustrated in Fig.~\ref{fig:schematic}.

%\begin{figure*}
%%%%%\begin{figure}
%%%%%	\centering
%%%%%%	\input{fig/schematicE}
%%%%%%	\includegraphics[scale=0.95]{fig/schematic}
%%%%%	\includegraphics[scale=0.75]{fig/schematic}
%%%%%%	\includegraphics[scale=0.75]{SysModel/fig/schematic_arrow}
%%%%%	\caption{Broadcasting an equiprobable binary source over an erasure broadcast channel.}
%%%%%	\label{fig:schematic}
%%%%%%\end{figure*}
%%%%%\end{figure}

%The problem is illustrated in Fig.~\ref{fig:schematic}.  
The problem is illustrated in Figure~\ref{fig:system_model_one_sided}.  The problem involving \emph{one-sided} feedback is a variation of the problem defined in Section~\ref{sec:system_model_feedback} with the exception that of the two receivers in the broadcast network, only the receiver with the lower erasure rate has a feedback channel available.  That is, at time $T$, we assume that only $\{Z_1(t)\}_{t=1, 2, \ldots, T-1}$ is available to the transmitter and both receivers rather than having $\{Z_1(t), Z_2(t)\}_{t=1, 2, \ldots, T-1}$ available.  We therefore redefine 

We consider the problem of communicating a binary memoryless source $\{S(t)\}_{t=1,2, \ldots}$ to two users over an erasure broadcast channel with one-sided feedback.  Of the two receivers in the broadcast network, only the receiver with the lower erasure rate has a feedback channel available. %Let $\mathcal{S}^{N}$ be the set of all $N$-vectors with components in $\mathcal{S}$, and denote $(S(1), S(2), \ldots , S(N))$ as $S^{N}$.  For convenience, we will also denote the set $\{1,2,\dots,N\}$ as $[N]$.
%
\begin{figure}
	\centering
%	\input{3/fig/schematic}
%	\includegraphics[scale=0.8]{3/one_sided/fig/system_model_one_sided}
	\includegraphics[scale=1]{one_sided/fig/system_model_one_sided}
%%	\includegraphics[width=0.6\textwidth]{outer_bound.png}
	\caption{Broadcasting an equiprobable binary source over an erasure broadcast channel with a feedback channel asymmetrically available to only the stronger user.}
	\label{fig:system_model_one_sided}
\end{figure}
%
The source produces equiprobable symbols in $\mathcal{S}=\{0,1\}$ and is communicated by an encoding function that produces the channel input sequence $X^{W} = (X(1),  \dots , X(W))$, where $X(t)$ denotes the $t^{\mathrm{th}}$ channel input taken from the alphabet $\mathcal{X} = \{0, 1\}$.  We assume that 
$X(t)$ is a function of the source as well as the channel outputs of the stronger user prior to time $t$.  
%The encoding function produces the channel input sequence $X^{W} = (X(1),  \dots , X(W))$, where $X(t)$ denotes the $t^{\mathrm{th}}$ channel input taken from the alphabet $\mathcal{X} = \{0, 1\}$.  %Note here that our notation defines $X^{n}$ as the first $n$ channel symbols sent. %which is also taken from the alphabet $\mathcal{S}$.  %

% Original
%Let $Y_{i}(t)$ be the channel output observed by user $i$ on the $t^{\mathrm{th}}$ channel use for $i \in [n]$ and $t \in [W]$.  Our channel model is an erasure channel.  In particular, let $\epsilon_i$ denote the erasure rate of the channel corresponding to user~$i$.  Without loss of generality, we will assume that $0 < \epsilon_{1} < \epsilon_{2} < \ldots < \epsilon_{n} < 1$.  Then $Y_{i}(t)$ exactly reproduces the channel input $X(t)$ with probability $(1 - \epsilon_i)$ and otherwise indicates an erasure event, which happens with probability $\epsilon_i$.  We let $Y_{i}(t)$ take on values in the alphabet $\mathcal{Y} = \{0, 1, \star\}$ so that an erasure event is represented by `$\star$,' the erasure symbol.  We associate user~$i$ with the state sequence $(N_i(t))_{t \in [W]}$, which is defined such that $N_{i}(t) = 1$ if $Y_i(t)$ was erased and $N_i(t) = 0$ otherwise.  The channel we consider is memoryless in the sense that $N_{i}(t)$ is drawn i.i.d.\ from a $\operatorname{Bern}(1 - \epsilon_{i})$ distribution.

Let $Y_{i}(t)$ be the channel output observed by user $i$ on the $t^{\mathrm{th}}$ channel use for $i \in \{1, 2\}$. %$\mathcal{U}= \{1, 2, 3\}$ and $t \in [W] = \{1, \ldots, W\}$.  %Our channel model is a binary erasure broadcast channel. % as shown in Fig.~\ref{fig:schematic}.  
%In particular, let $\epsilon_i$ denote the erasure rate of the channel corresponding to user~$i$, where we assume that $0 < \epsilon_{1} < \epsilon_{2} < \ldots < \epsilon_{n} < 1$.  This is without loss of generality since we can address {{}all} users that experience identical erasure rates by serving the {{}one} with the most stringent distortion requirement.  
%In particular, if $\epsilon_i$ denotes the erasure rate of the channel corresponding to user~$i$, our model specifies that $Y_{i}(t)$ exactly reproduces the channel input $X(t)$ with probability $(1 - \epsilon_i)$ and otherwise indicates an erasure event, which happens with probability $\epsilon_i$.  
We let $Y_{i}(t)$ take on values in the alphabet $\mathcal{Y} = \{0, 1, \star\}$ so that an erasure event is represented by `$\star$'.   
%
We associate user~$i$ with the state sequence $\{Z_i(t)\}_{t \in [W]}$, which represents the noise on user~$i$'s channel, where $Z_i(t) \in \mathcal{Z} = \{0,1\}$,  and  $Y_i(t)$ will be erased if $Z_{i}(t) = 1$ and $Y_{i}(t) = X(t)$ if $Z_i(t) = 0$.  The channel we consider is memoryless in the sense that $(Z_{1}(t), Z_2(t))$ is drawn i.i.d.\ from the probability mass function given by   
%For $i, j \in \{1, 2\}$, let $p_{E}(i, j) = \textrm{Pr}(Z_1(t) = i - 1, Z_2(t) = j - 1)$, and let $P_{E} \in \mathbb{R}^{2 \times 2}$ be the stochastic matrix such that $P_{E} = [p_{E}(i, j)]$

\begin{subequations}
\label{eq:pmf_z1z2}
\begin{align}
	\textrm{Pr}(Z_1 = 1, Z_2 = 1) &= \epsot \\
	\textrm{Pr}(Z_1 = 1, Z_2 = 0) &= \epsilon_1 - \epsot \\
	\textrm{Pr}(Z_1 = 0, Z_2 = 1) &= \epsilon_2 - \epsot \\
	\textrm{Pr}(Z_1 = 0, Z_2 = 0) &= 1 - \epsilon_1 - \epsilon_2 + \epsot,			
\end{align}
\end{subequations}
where $\epsot\in (0, 1)$ is the probability that an erasure simultaneously occurs on both channels and $\epsilon_i \in (0, 1)$ denotes the erasure rate of the channel corresponding to user~$i$, where we assume $\epsilon_1 < \epsilon_2$.
%$\epsilon_i$ denotes the erasure rate of the channel corresponding to user~$i$, and we assume $\epsilon_1 < \epsilon_2$.
%\textcolor{blue}{We assume that the erasure rates are known to both the transmitter and receiver. If such channel knowledge is not possible, we can take the standard approach of interpreting a broadcast channel as an abstraction for a \emph{compound channel}~\cite{CT}.  In such a situation, the compound channel is a channel that randomly takes on one of many potential states for the duration of transmission.  We model this by considering a broadcast channel whose constituent channels correspond to these potential channel states.}
%{}{Note that in our setup, the erasure rates for each user are assumed to be known. However, our setup also models the 
%compound channel~\cite{CT}, where an erasure rate is not known and instead belong to a collection of possible states, with each 
%state corresponding to one virtual user in our system.}

%Let $Y_{i}(t)$ be the channel output observed by user $i$ on the $t^{\mathrm{th}}$ channel use for $i \in [n]$ and $t \in [W]$.  Our channel model is an erasure channel.  In particular, $Y_{i}(t)$ either exactly reproduces the channel input $X(t)$ or otherwise indicates an erasure event.  We let $Y_{i}(t)$ take on values in the alphabet $\mathcal{Y} = \{0, 1, \star\}$ so that an erasure event is represented by `$\star$,' the erasure symbol.  Let $\epsilon_i$ denote the erasure rate of the channel corresponding to user~$i$.  Without loss of generality, we assume that $0 < \epsilon_{1} < \epsilon_{2} < \ldots < \epsilon_{n} < 1$.  We associate user~$i$ with the state sequence $(N_i(t))_{t \in [W]}$, where $N_i(t) \in \{0,1\}$.  The state sequence represents the noise on user~$i$'s channel and we will have that $Y_i(t)$ is erased if $N_{i}(t) = 1$ and $Y_{i}(t) = X(t)$ if $N_i(t) = 0$.  The channel we consider is memoryless in the sense that $N_{i}(t)$ is drawn i.i.d.\ from a $\operatorname{Bern}(1 - \epsilon_{i})$ distribution.

%\begin{equation}
%%\label{eq:channel_model}
%	Y_{i}(t) = X(t) \cdot N_{i}(t),
%\end{equation}
%
%where $N_{i}(l)$ is a $\operatorname{Bern}(1 - \epsilon_{i})$ random variable representing the noise at user $i$'s $l^{\mathrm{th}}$ channel output.  The channel is memoryless in the sense that $N_{i}(l)$ is drawn i.i.d.\ from a $\operatorname{Bern}(1 - \epsilon_{i})$ distribution.  %Specifically, the statistics of $N_{i}(l)$ are such that
%
%\begin{equation}
%\label{eq:nstat}
%	N_{i}(l) =
%	\begin{cases}
%		0 & \text{with probability} \ \epsilon_{i}, \\
%		1 & \text{with probability} \ 1 - \epsilon_{i}.
%	\end{cases}
%\end{equation}
%
%Thus, $Y_{i}(l)$ takes on values in the alphabet $\mathcal{Y} = \{-1, 0, +1\}$ and we interpret $Y_{i}(l)$ as the output of an erasure channel, with erasure probability $\epsilon_{i}$, when $X(l)$ is the channel input (see Section~\ref{sec:erased_rv} for a discussion of the erasure channel model).
%
%Thus, $Y_{i}(l)$ takes on values in the alphabet $\mathcal{Y} = \{-1, 0, +1\}$.  If we define `0' as the erasure symbol, we can interpret $Y_{i}(l)$ as the output of an erasure channel with erasure probability $\epsilon_{i}$ when $X(l)$ is the channel input. Without loss of generality, we will assume that $0 < \epsilon_{1} < \epsilon_{2} < \ldots < \epsilon_{n} < 1$. %Users on channels with the same erasure probability are represented by a user of the smallest distortion

%Now although the length-$n$ channel input is broadcasted to both users, we will assume that due to each user's delay constraint, the $i^{\mathrm{th}}$ user reconstructs the source after observing only the first $n_{i}$ channel input symbols, denoted as $X^{n_{i}}$, where $n_{i} \leq n$.  Specifically, we have that $n = \max(n_{1}, n_{2})$.

The problem we consider involves causal feedback from the stronger user that is universally available.  That is, at time $T$, we assume that $\{Z_1(t)\}_{t=1, 2, \ldots, T-1}$ is available to the transmitter and both receivers. 
After $W$ channel uses, user $i$ utilizes the feedback and his own channel output to reconstruct the source as a length-$N$ sequence, denoted as $\hat{S}_{i}^{N}$.  We will be interested in a fractional recovery requirement so that each symbol in $\hat{S}_{i}^{N}$ either faithfully recovers the corresponding symbol in $S^{N}$, or otherwise a failure is indicated with an erasure symbol, i.e., we do not allow for any bit flips.

More precisely, we choose the reconstruction alphabet $\mathcal{\hat{S}}$ to be an augmented version of the source alphabet so that $\mathcal{\hat{S}} = \{0, 1, \star\}$, where the additional `$\star$' symbol indicates an erasure symbol.  Let $\mathcal{D} = [0,1]$ and $d_i \in \mathcal{D}$ be the distortion user $i$ requires.  We then express the constraint that an achievable code ensures that each user $i \in \{1, 2\}$ achieves a fractional recovery of $1 - d_{i}$ with the following definition.

%by first defining the set $D_{i}(\hat{S}_{i}^{N}) = \{l \in [N] : \hat{S}_{i}(l) = 0\}$.

%Note that the we have taken the reconstruction alphabet to be an augmented version of the source alphabet by adding the additional `0' symbol, which we interpret as an erasure symbol.  In our reconstruction, we require that $\hat{S}_{i}^{N}$ is such that for $l \in [N]$, $\hat{S}_{i}(l) = S(l)$ or $\hat{S}_{i}(l) = 0$.  In other words, we do not allow any bit flips in our reconstruction so that $\hat{S}_{i}(l)$ either faithfully reproduces $S(l)$ or otherwise outputs an erasure symbol.


%%%On a symbol-by-symbol basis, we measure the reconstruction's fidelity with the erasure distortion $d_{E}: \mathcal{S} \times \hat{\mathcal{S}} \to \{0,1, \infty\}$ given by
%%%%Depending on the distortion measure we use, $\mathcal{\hat{S}}$ can either be a binary source alphabet or the extended alphabet $\mathcal{\hat{S}_{E}} = \{-1, 0, 1\}$, where `0' denotes the source erasure symbol.
%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%On the other hand, when the output alphabet can include the source erasure symbol as in the second case, then on a symbol-by-symbol comparison, the reconstruction's fidelity is measured with the erasure distortion $d_{E} : \mathcal{S} \times \mathcal{\hat{S}_{E}} \to \{0, 1, \infty\}$, given by
%%%
%%%\begin{equation}
%%%\label{eq:symbol_distortion1}
%%%	d_{E}(s, \hat{s}) =
%%%	\begin{cases}
%%%		0 & \text{if } \hat{s} = s, \\
%%%		1 & \text{if } \hat{s} = 0 \\
%%%		\infty & \text{otherwise}.
%%%	\end{cases}
%%%\end{equation}
%%%%
%%%The per-letter distortion of a vector is then defined as $d(s^{k}, \hat{s}^{k}) = \frac{1}{k} \Sigma_{m=1}^{k} d(s_{m}, \hat{s}_{m})$.
%%%
%%%%\begin{equation}
%%%%\label{eq:vector_distortion1}
%%%%	d(s^{k}, \hat{s}^{k}) = \frac{1}{k} \sum\limits_{i=1}^k d(s_{i}, \hat{s}_{i}).
%%%%\end{equation}
%%%%
%%%%where $d(\cdot, \cdot)$ can be either $d_{H}(\cdot, \cdot)$ or $d_{E}(\cdot, \cdot)$.
%%%
%%%%We point out that with the erasure distortion measure,  a finite distortion value indicates that we are certain about the accuracy of the non-erased symbols in our reconstruction, while the actual value of the distortion is a measure of the proportion of bits that we are unsure about, i.e., that have been erased in the reconstruction.
%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
%%%
%%%We point out that with the erasure distortion measure,  a finite distortion value indicates that we are certain about the accuracy of the non-erased symbols in our reconstruction, while the actual value of the distortion is a measure of the proportion of bits that we are unsure about, i.e., that have been erased in the reconstruction.  We now define the components of our problem.

\begin{mydef}
\label{def:code_one_sided}
	An $(N, W, d_{1}, d_{2})$ code for source $S$ on the erasure broadcast channel with \emph{one-sided} feedback consists of	
	\begin{enumerate}
		\item A sequence of encoding functions $f_{i, N} : \mathcal{S}^{N} \times  \mathcal{Z}^{i-1} \to \mathcal{X}$ for $i \in [W]$, s.t.\ $X(i) = f_{i, N}(S^{N}, Z_1^{i -1})$
		
		\item Two decoding functions $g_{i,N} : \mathcal{Y}^{W} \times \mathcal{Z}^{W} \to \mathcal{\hat{S}}^{N}$ s.t.\ $\hat{S}_{i}^{N} = g_{i,N}(Y_{i}^{W}, Z_1^{W})$, $i \in \{1, 2\}$, and
		\begin{enumerate}
			\item $\hat{S}_{i}^{N}$ is such that for $t \in [N]$, if $\hat{S}_{i}(t) \neq S(t)$, then $\hat{S}_{i}(t) = \star$,
%			\item $\mathbb{E}   \left\vert{D_{i}(\hat{S}_{i}^{N})}\right\vert \leq d_{i}$
			\item $\mathbb{E}   \left\vert{\{t \in [N] \mid \hat{S}_{i}(t) = \star\}}\right\vert \leq N d_{i}$,
		\end{enumerate}
		 	
%	$\mathbb{E}d(S^{k}, g_{i}( X^{n} \cdot N_{i}^{n})) \leq D_{i}$ holds for $i \in \{1,2\}$		
	\end{enumerate}
	
%	where $\mathbb{E}(\cdot)$ is the expectation operation and $\vert A \vert$ denotes the cardinality of set $A$.
\end{mydef}

%\begin{mydef}
%\label{def:code}
%	An $(N, W, d_{1}, d_{2}, d_{3})$ code for source $S$ on the erasure broadcast channel consists of
%	\begin{enumerate}
%		\item a sequence of encoding functions $f_{i, N} : \mathcal{S}^{N} \times  \prod_{j = 1}^{3} \mathcal{N}^{i-1} \to \mathcal{X}$ for $i \in [W]$, such that $X(i) = f_{i, N}(S^{N}, N_1^{i -1}, N_2^{i -1}, N_3^{i - 1})$, and
%		
%		\item three decoding functions $g_{i,N} : \mathcal{Y}^{W} \times  \prod_{j = 1}^{3} \mathcal{N}^{W} \to \mathcal{\hat{S}}^{N}$ s.t.\ $\hat{S}_{i}^{N} = g_{i,N}(Y_{i}^{W}, N_1^{W}, N_2^{W}, N_3^{W})$, $i \in \{1, 2, 3\}$,
%		\begin{enumerate}
%			\item $\hat{S}_{i}^{N}$ is such that for $t \in [N]$, if $\hat{S}_{i}(t) \neq S(t)$, then $\hat{S}_{i}(t) = \star$,
%%			\item $\mathbb{E}   \left\vert{D_{i}(\hat{S}_{i}^{N})}\right\vert \leq d_{i}$
%			\item $\mathbb{E}   \left\vert{\{t \in [N] \mid \hat{S}_{i}(t) = \star\}}\right\vert \leq N d_{i}$,
%		\end{enumerate}
%		 	
%%	$\mathbb{E}d(S^{k}, g_{i}( X^{n} \cdot N_{i}^{n})) \leq D_{i}$ holds for $i \in \{1,2\}$		
%	\end{enumerate}
%	
%%	where $\mathbb{E}(\cdot)$ is the expectation operation and $\vert A \vert$ denotes the cardinality of set $A$.
%\end{mydef}

%A point is now made about the modelling of latencies in our problem.  We define the \emph{latency} or \emph{bandwidth expansion factor} $b \in [0, \infty )$, as the number of channel uses per source symbol that are delivered over the broadcast channel, i.e., $b \triangleq n/k$.  This is to say that $b \cdot k$ channel uses are required before both users can reconstruct $S^{k}$ subject to their distortion constraints.  Our problem is now defined as characterizing the achievable latency region under a given pair of distortion constraints as per the next definition.

%A point is now made about the modelling of delays in our problem.  We define the bandwidth expansion factor $b \in [0, \infty )$, as $b = n/k$.  We interpret $b$ as the normalized latency (in units of ``channel uses per source symbol''), before both users can reconstruct $S^{k}$ subject to their distortion constraints.  Our problem is now defined as characterizing the achievable distortion region under a given bandwidth expansion factor as per the next definition.
%
We next define the {\it latency} that a given code requires before all users can recover their desired fraction of the source.
\begin{mydef}
	The latency, $w$, of an~$(N, W, d_{1}, d_{2})$ code is the number of channel uses per source symbol that the code requires to meet all distortion demands, i.e., $w = W/N$.
\end{mydef}
%
Our goal is to characterize the achievable latencies under a prescribed distortion vector,
as per the following definition.
\begin{mydef}
\label{def:achievable_one_sided}
	Latency $w$ is said to be $(d_{1}, d_{2})$-achievable over the erasure broadcast channel with one-sided feedback if for every $\delta > 0$, there exists for sufficiently large $N$, an $(N, wN, \hat{d}_{1}, \hat{d}_{2})$ code such that for all $i \in \{1, 2\}$, $d_{i}+\delta \geq \hat{d}_{i}$.
	
%	\begin{equation}
%		D_{i}+\delta \geq d_{i},  \quad i \in \{1, 2\}.
%	\end{equation}	
%	Alternatively, we may occasionally say that the tuple $(b, D_{1}, D_{2})$ is achievable if the latency $b$ is $(D_{1}, D_{2})$-achievable.
	
%The achievable latency region is the set of all achievable latencies under the prescribed distortion vector.

\end{mydef}

%In the remaining sections, we consider the cases $n=2$ and $n=3$.  We will also make a mention whenever the strategies we use for these cases can be generalized for $n$ users.  
%While this may seem to be an oversimplification, it is worth noting that to the authors' best knowledge, a solution is also not known for the related channel coding problem involving $n$ users~\cite{GGT}.

%\begin{remark}
%\label{rem:deps}
%Throughout this paper we will assume that for each user $i \in [n]$, we have that $d_i < \epsilon_i$. Any user with $d_i \ge \epsilon_i$ will be trivially satisfied by the systematic portion of our segmentation-based coding scheme.  Furthermore, we will show in Lemma~\ref{lem:bn1} that within our class of coding schemes, such a systematic portion can be transmitted without loss of optimality when at least one user satisfies $d_i < \epsilon_i$. Finally, if every user satisfies $d_i \ge \epsilon_i$, a simple uncoded transmission scheme is easily shown to be optimal.
%\end{remark}
%
%\begin{remark}
%	While our system model has assumed binary alphabets for both the source and channel input sequences, our results can be easily extended to larger alphabet sizes for the purpose of applying our results to packet erasure networks.
%\end{remark}


%For convenience, throughout this paper, for any positive integer $k$, we shorthand the set $\{1,2,\dots,k\}$ as $[k].$
%
%Consider broadcasting a length-$N$ binary sequence $S = \{s(j)\}_{j\in[N]}$ from a source to $n$ receivers over independent memoryless binary erasure channels. For $i\in[n]$, denote the erasure rate of the channel between the source and receiver $i$ as $\epsilon_i$. Applying some encoding scheme to $S$, the source generates and broadcasts the coded binary sequence $X=\{x_j\}_{j\ge1}$. Each receiver $i$ retrieves from the channel a sequence $Y^i = \{y_{j}^i\}_{j\ge1}$ where $y_{j}^i \in \{0,1,e\}$, $e$ indicating an erasure. Denote $Y^{i,W} = \{y_{j}^i\}_{j\in[W]}$ as the truncation of $Y^i$ up to the $W$th symbol. Receiver $i$ reconstructs from $Y^{i,W}$ a copy $\hat S^{i,W}=\{\hat s_{j}^{i,W}\}_{j\in[N]},$ where $\hat s_{j}^{i,W}\in\{0,1,e\}.$
%
%%\subsection{Erasure Distortion}
%We consider a symbol-by-symbol based erasure reconstruction distortion measure $D_e: \{0,1\}\times \{0,1,e\}\mapsto \mathds R$ defined as
%\begin{align*}
%D_E(s,\hat s) = \left\{\begin{array}{lr} 0,& \textnormal{if } \hat s=s\\ 1, & \textnormal{if } \hat s\ne s, \hat s\ne e\\ \infty,& \textnormal{if } \hat s=e \end{array}\right.
%\end{align*}
%%for symbols $s\in\{0,1\}$ and $\hat s\in\{0,1,e\}$,
%and
%\begin{align*}
%D(S,\hat S^{i,W}) =  \frac{1}{N}\sum_{j\in[N]} D_E(s_j,\hat s_{j}^{i,W}).
%\end{align*}
%for the source sequence $S$ and the sequence $\hat S^{i,W}$ reconstructed by user $i$ from the first $W$ symbols of the channel output sequence $Y^{i,W}$.
%
%Now our problem is to upper bound and lower bound the minimum $W$, or $w=W/N,$ which we refer to as the {\it latency}, that guarantees $\mathds E[ D(S,\hat S^{i,W})]\le d_i$ for all $i\in[n]$,
%where $d_i$ is the given distortion requirement of user $i$.
%
%Clearly, $w$ is trivially lower bounded by $\max_{i\in[n]}\{\frac{1-d_i}{1-\epsilon_i}\}$. In the next section, we provide an upper bound of $w$ and the achieving coding scheme. We show that the upper bound is achieved with a coding scheme that sends a part of the source sequence uncoded, partitions the rest of the source sequence into a number of segments, and encodes each segment by a systematic optimal erasure code. The optimal segmentation can be found by solving a linear programming problem. We also show in Sec.~\ref{sec:jscc} that the segmentation-based scheme is equivalent to the Mittal-Phamdo~\cite{} scheme for erasure channels.

%\input{SysModel/individual_code}




%\input{SysModel/JSCC_approach3}










==> problem_formulation.tex <==
\section{{}{System Model}}
%\subsection{{}System Model}
%\section{Problem Formulation}
\label{sec:system_model}

%We first define the problem in Section~\ref{subsec:problem_definition}.  In Section~\ref{subsec:metrics}, we then discuss metrics that are of interest in the evaluation of broadcast codes and show how a solution to the problem in Section~\ref{subsec:problem_definition} can be used to address these metrics.

%\input{2_problem_formulation/problem_definition}
%\input{2_problem_formulation/metrics}

%%%\begin{figure*}
%%\begin{figure}
%%	\centering
%%%	\input{3/out/fig/schematic}
%%%	\includegraphics[scale=0.6]{3/out/fig/schematica}
%%%	\includegraphics[scale=0.75]{out/fig/schematic}
%%%	\includegraphics[scale=0.8]{2_problem_formulation/fig/schematicE}
%%	\includegraphics{2_problem_formulation/fig/schematicE}
%%%	\includegraphics[width=0.6\textwidth]{outer_bound.png}
%%	\caption{Broadcasting an equiprobable binary source over an erasure broadcast channel.}
%%	\label{fig:schematic}
%%%\end{figure*}
%%\end{figure}

%We begin by presenting our joint source-channel coding formulation which is illustrated in Fig.~\ref{fig:schematic}.

%\begin{figure*}
\begin{figure}
	\centering
%	\input{fig/schematicE}
%	\includegraphics[scale=0.95]{fig/schematic}
%	\includegraphics[scale=0.75]{fig/schematicE_two_bec}
	\includegraphics[scale=1]{fig/schematicE_two_bec}
%	\includegraphics[scale=0.75]{SysModel/fig/schematic_arrow}
	\caption{Broadcasting an equiprobable binary source over an erasure broadcast channel.}
	\label{fig:schematic}
%\end{figure*}
\end{figure}

The problem is illustrated in Fig.~\ref{fig:schematic}.  We consider {{}a} binary memoryless source $\{S(t)\}_{t=1,2, \ldots}$ that produces equiprobable symbols in the alphabet $\mathcal{S}=\{0,1\}$ and that we wish to communicate to two users over an erasure broadcast channel.  %Let $\mathcal{S}^{N}$ be the set of all $N$-vectors with components in $\mathcal{S}$, and denote $(S(1), S(2), \ldots , S(N))$ as $S^{N}$.  For convenience, we will also denote the set $\{1,2,\dots,N\}$ as $[N]$.
%
%\begin{figure}
%	\centering
%%	\input{3/fig/schematic}
%	\includegraphics[scale=0.8]{fig/schematicE}
%%%	\includegraphics[width=0.6\textwidth]{outer_bound.png}
%	\caption{Broadcasting an equiprobable binary source over an erasure broadcast channel with individual bandwidth mismatches.}
%	\label{fig:schematicE}
%\end{figure}
%
The source is communicated by a block-encoding function that maps a length-$m$ source sequence, $S^{m}$, to a length-$n$ channel input sequence, $X^{n} = (X(1), X(2), \ldots , X(n))$, where $X(t)$ denotes the $t^{\mathrm{th}}$ channel input taken from the alphabet $\mathcal{X} = \{0, 1\}$.  %Note here that our notation defines $X^{n}$ as the first $n$ channel symbols sent. %which is also taken from the alphabet $\mathcal{S}$.  %

% Original
%Let $Y_{i}(t)$ be the channel output observed by user $i$ on the $t^{\mathrm{th}}$ channel use for $i \in [n]$ and $t \in [W]$.  Our channel model is an erasure channel.  In particular, let $\epsilon_i$ denote the erasure rate of the channel corresponding to user~$i$.  Without loss of generality, we will assume that $0 < \epsilon_{1} < \epsilon_{2} < \ldots < \epsilon_{n} < 1$.  Then $Y_{i}(t)$ exactly reproduces the channel input $X(t)$ with probability $(1 - \epsilon_i)$ and otherwise indicates an erasure event, which happens with probability $\epsilon_i$.  We let $Y_{i}(t)$ take on values in the alphabet $\mathcal{Y} = \{0, 1, \star\}$ so that an erasure event is represented by `$\star$,' the erasure symbol.  We associate user~$i$ with the state sequence $(N_i(t))_{t \in [W]}$, which is defined such that $N_{i}(t) = 1$ if $Y_i(t)$ was erased and $N_i(t) = 0$ otherwise.  The channel we consider is memoryless in the sense that $N_{i}(t)$ is drawn i.i.d.\ from a $\operatorname{Bern}(1 - \epsilon_{i})$ distribution.

Let $Y_{i}(t)$ be the channel output observed by user $i$ on the $t^{\mathrm{th}}$ channel use for $i \in \{1, 2\}$ and $t \in [n]$.  Our channel model is a binary erasure broadcast channel as shown in Fig.~\ref{fig:schematic}.  In particular, let $\epsilon_i$ denote the erasure rate of the channel corresponding to user~$i$, where we assume that $0 < \epsilon_{1} < \epsilon_{2}$, and $\epsilon_2 = 1 - 1/M$ for some integer $M > 1$.  Our model specifies that $Y_{i}(t)$ exactly reproduces the channel input $X(t)$ with probability $(1 - \epsilon_i)$ and otherwise indicates an erasure event, which happens with probability $\epsilon_i$.  We let $Y_{i}(t)$ take on values in the alphabet $\mathcal{Y} = \{0, 1, \star\}$ so that an erasure event is represented by `$\star$,' the erasure symbol.  
We can associate user~$i$ with the channel-noise state sequence $(N_i(t))_{t \in [n]}$, where $N_i(t) \in \{0,1\}$, and we will have that $Y_i(t)$ is erased if $N_{i}(t) = 1$ and $Y_{i}(t) = X(t)$ if $N_i(t) = 0$.  The channel we consider is memoryless in the sense that $N_{i}(t)$ is drawn i.i.d.\ from a $\operatorname{Bern}(\epsilon_{i})$ distribution.
%\textcolor{blue}{We assume that the erasure rates are known to both the transmitter and receiver. If such channel knowledge is not possible, we can take the standard approach of interpreting a broadcast channel as an abstraction for a \emph{compound channel}~\cite{CT}.  In such a situation, the compound channel is a channel that randomly takes on one of many potential states for the duration of transmission.  We model this by considering a broadcast channel whose constituent channels correspond to these potential channel states.}
%{}{Note that in our setup, the erasure rates for each user are assumed to be known. However, our setup also models the 
%compound channel~\cite{CT}, where the erasure rate is not known and instead belong to a collection of possible states, with each 
%state corresponding to one virtual user in our system.}

%Let $Y_{i}(t)$ be the channel output observed by user $i$ on the $t^{\mathrm{th}}$ channel use for $i \in [n]$ and $t \in [W]$.  Our channel model is an erasure channel.  In particular, $Y_{i}(t)$ either exactly reproduces the channel input $X(t)$ or otherwise indicates an erasure event.  We let $Y_{i}(t)$ take on values in the alphabet $\mathcal{Y} = \{0, 1, \star\}$ so that an erasure event is represented by `$\star$,' the erasure symbol.  Let $\epsilon_i$ denote the erasure rate of the channel corresponding to user~$i$.  Without loss of generality, we assume that $0 < \epsilon_{1} < \epsilon_{2} < \ldots < \epsilon_{n} < 1$.  We associate user~$i$ with the state sequence $(N_i(t))_{t \in [W]}$, where $N_i(t) \in \{0,1\}$.  The state sequence represents the noise on user~$i$'s channel and we will have that $Y_i(t)$ is erased if $N_{i}(t) = 1$ and $Y_{i}(t) = X(t)$ if $N_i(t) = 0$.  The channel we consider is memoryless in the sense that $N_{i}(t)$ is drawn i.i.d.\ from a $\operatorname{Bern}(1 - \epsilon_{i})$ distribution.

%\begin{equation}
%%\label{eq:channel_model}
%	Y_{i}(t) = X(t) \cdot N_{i}(t),
%\end{equation}
%
%where $N_{i}(l)$ is a $\operatorname{Bern}(1 - \epsilon_{i})$ random variable representing the noise at user $i$'s $l^{\mathrm{th}}$ channel output.  The channel is memoryless in the sense that $N_{i}(l)$ is drawn i.i.d.\ from a $\operatorname{Bern}(1 - \epsilon_{i})$ distribution.  %Specifically, the statistics of $N_{i}(l)$ are such that
%
%\begin{equation}
%\label{eq:nstat}
%	N_{i}(l) =
%	\begin{cases}
%		0 & \text{with probability} \ \epsilon_{i}, \\
%		1 & \text{with probability} \ 1 - \epsilon_{i}.
%	\end{cases}
%\end{equation}
%
%Thus, $Y_{i}(l)$ takes on values in the alphabet $\mathcal{Y} = \{-1, 0, +1\}$ and we interpret $Y_{i}(l)$ as the output of an erasure channel, with erasure probability $\epsilon_{i}$, when $X(l)$ is the channel input (see Section~\ref{sec:erased_rv} for a discussion of the erasure channel model).
%
%Thus, $Y_{i}(l)$ takes on values in the alphabet $\mathcal{Y} = \{-1, 0, +1\}$.  If we define `0' as the erasure symbol, we can interpret $Y_{i}(l)$ as the output of an erasure channel with erasure probability $\epsilon_{i}$ when $X(l)$ is the channel input. Without loss of generality, we will assume that $0 < \epsilon_{1} < \epsilon_{2} < \ldots < \epsilon_{n} < 1$. %Users on channels with the same erasure probability are represented by a user of the smallest distortion

%Now although the length-$n$ channel input is broadcasted to both users, we will assume that due to each user's delay constraint, the $i^{\mathrm{th}}$ user reconstructs the source after observing only the first $n_{i}$ channel input symbols, denoted as $X^{n_{i}}$, where $n_{i} \leq n$.  Specifically, we have that $n = \max(n_{1}, n_{2})$.

Having observed his channel output, user $i$ then uses it to reconstruct the source as a length-$m$ sequence, denoted as $\hat{S}_{i}^{m}$.  We will be interested in a fractional recovery requirement so that each symbol in $\hat{S}_{i}^{m}$ either faithfully recovers the corresponding symbol in $S^{m}$, or otherwise a failure is indicated with an erasure symbol, i.e., we do not allow for any bit flips.

More precisely, we choose the reconstruction alphabet $\mathcal{\hat{S}}$ to be an augmented version of the source alphabet so that $\mathcal{\hat{S}} = \{0, 1, \star\}$, where the additional `$\star$' symbol indicates an erasure symbol.  We then express the constraint that an achievable code ensures that each user $i \in \{1, 2\}$ achieves a fractional recovery of $1 - d_{i}$, where $d_{i}  \in [0, 1]$, with the following definition.




%by first defining the set $D_{i}(\hat{S}_{i}^{N}) = \{l \in [N] : \hat{S}_{i}(l) = 0\}$.

%Note that the we have taken the reconstruction alphabet to be an augmented version of the source alphabet by adding the additional `0' symbol, which we interpret as an erasure symbol.  In our reconstruction, we require that $\hat{S}_{i}^{N}$ is such that for $l \in [N]$, $\hat{S}_{i}(l) = S(l)$ or $\hat{S}_{i}(l) = 0$.  In other words, we do not allow any bit flips in our reconstruction so that $\hat{S}_{i}(l)$ either faithfully reproduces $S(l)$ or otherwise outputs an erasure symbol.


%%%On a symbol-by-symbol basis, we measure the reconstruction's fidelity with the erasure distortion $d_{E}: \mathcal{S} \times \hat{\mathcal{S}} \to \{0,1, \infty\}$ given by
%%%%Depending on the distortion measure we use, $\mathcal{\hat{S}}$ can either be a binary source alphabet or the extended alphabet $\mathcal{\hat{S}_{E}} = \{-1, 0, 1\}$, where `0' denotes the source erasure symbol.
%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%On the other hand, when the output alphabet can include the source erasure symbol as in the second case, then on a symbol-by-symbol comparison, the reconstruction's fidelity is measured with the erasure distortion $d_{E} : \mathcal{S} \times \mathcal{\hat{S}_{E}} \to \{0, 1, \infty\}$, given by
%%%
%%%\begin{equation}
%%%\label{eq:symbol_distortion1}
%%%	d_{E}(s, \hat{s}) =
%%%	\begin{cases}
%%%		0 & \text{if } \hat{s} = s, \\
%%%		1 & \text{if } \hat{s} = 0 \\
%%%		\infty & \text{otherwise}.
%%%	\end{cases}
%%%\end{equation}
%%%%
%%%The per-letter distortion of a vector is then defined as $d(s^{k}, \hat{s}^{k}) = \frac{1}{k} \Sigma_{m=1}^{k} d(s_{m}, \hat{s}_{m})$.
%%%
%%%%\begin{equation}
%%%%\label{eq:vector_distortion1}
%%%%	d(s^{k}, \hat{s}^{k}) = \frac{1}{k} \sum\limits_{i=1}^k d(s_{i}, \hat{s}_{i}).
%%%%\end{equation}
%%%%
%%%%where $d(\cdot, \cdot)$ can be either $d_{H}(\cdot, \cdot)$ or $d_{E}(\cdot, \cdot)$.
%%%
%%%%We point out that with the erasure distortion measure,  a finite distortion value indicates that we are certain about the accuracy of the non-erased symbols in our reconstruction, while the actual value of the distortion is a measure of the proportion of bits that we are unsure about, i.e., that have been erased in the reconstruction.
%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
%%%
%%%We point out that with the erasure distortion measure,  a finite distortion value indicates that we are certain about the accuracy of the non-erased symbols in our reconstruction, while the actual value of the distortion is a measure of the proportion of bits that we are unsure about, i.e., that have been erased in the reconstruction.  We now define the components of our problem.

\begin{mydef}
\label{def:code}
	An $(m, n, d_{1}, d_{2})$ code for source $S$ on the erasure broadcast channel consists of
	
	\begin{enumerate}
		\item an encoding function $f_{m} : \mathcal{S}^{m} \to \mathcal{X}^{n}$ such that $X^{n} = f_{m}(S^{m})$, and
		
		\item Two decoding functions $g_{i,m} : \mathcal{Y}^{n} \to \mathcal{\hat{S}}^{m}$ such that $\hat{S}_{i}^{m} = g_{i,m}(Y_{i}^{n})$ and for each $i \in \{1, 2\}$,
		\begin{enumerate}
			\item $\hat{S}_{i}^{m}$ is such that for $t \in [m]$, if $\hat{S}_{i}(t) \neq S(t)$, then $\hat{S}_{i}(t) = \star$,
%			\item $\mathbb{E}   \left\vert{D_{i}(\hat{S}_{i}^{N})}\right\vert \leq d_{i}$
			\item $\mathbb{E}   \left\vert{\{t \in [m] \mid \hat{S}_{i}(t) = \star\}}\right\vert \leq m d_{i}$,
		\end{enumerate}
		 	
%	$\mathbb{E}d(S^{k}, g_{i}( X^{n} \cdot N_{i}^{n})) \leq D_{i}$ holds for $i \in \{1,2\}$		
	\end{enumerate}
	
	where $\mathbb{E}(\cdot)$ is the expectation operation and $\vert A \vert$ denotes the cardinality of set $A$.
\end{mydef}

\begin{remark}
	The fractional recovery requirement of our problem can also be captured by considering the erasure distortion $d_{E}(\cdot, \cdot)$, and requiring that the average $m$-letter distortion between the source and reconstruction sequences be less than a prescribed value.   For $s \in \mathcal{S}$, and $\hat{s} \in \mathcal{\hat{S}}$, the erasure distortion measure is given by
\begin{equation}
\label{eq:symbol_distortion1}
	d_{E}(s, \hat{s}) =
	\begin{cases}
		0 & \text{if } \hat{s} = s, \\
		1 & \text{if } \hat{s} = \star \\
		\infty & \text{otherwise}.
	\end{cases}
\end{equation}

\end{remark}

%A point is now made about the modelling of latencies in our problem.  We define the \emph{latency} or \emph{bandwidth expansion factor} $b \in [0, \infty )$, as the number of channel uses per source symbol that are delivered over the broadcast channel, i.e., $b \triangleq n/k$.  This is to say that $b \cdot k$ channel uses are required before both users can reconstruct $S^{k}$ subject to their distortion constraints.  Our problem is now defined as characterizing the achievable latency region under a given pair of distortion constraints as per the next definition.

%A point is now made about the modelling of delays in our problem.  We define the bandwidth expansion factor $b \in [0, \infty )$, as $b = n/k$.  We interpret $b$ as the normalized latency (in units of ``channel uses per source symbol''), before both users can reconstruct $S^{k}$ subject to their distortion constraints.  Our problem is now defined as characterizing the achievable distortion region under a given bandwidth expansion factor as per the next definition.

For a given code, we next define the {\it latency} that the code requires before all users can recover their desired fraction of the source.  We then state our problem as characterizing the achievable distortion pairs under a prescribed latency as per the following definitions.

\begin{mydef}
	The latency, $b$, of an~$(m, n, d_{1}, d_{2})$ code is the number of channel uses per source symbol that the code requires to meet all distortion demands, i.e., $b = n/m$.
\end{mydef}

\begin{mydef}
\label{def:achievable}
	The distortion pair $(d_{1}, d_{2})$ is said to be achievable with latency $b$ over the erasure broadcast channel if for every $\delta > 0$, there exists for sufficiently large $m$, an $(m, b\cdot m, \hat{d}_{1}, \hat{d}_{2})$ code such that for all $i \in \{1, 2\}$, $d_{i}+\delta \geq \hat{d}_{i}$.
\end{mydef}

%\begin{mydef}
%\label{def:achievable}
%	Latency $b$ is said to be $(d_{1}, d_{2})$-achievable over the erasure broadcast channel if for every $\delta > 0$, there exists for sufficiently large $m$, an $(m, b\cdot m, \hat{d}_{1}, \hat{d}_{2})$ code such that for all $i \in \{1, 2\}$, $d_{i}+\delta \geq \hat{d}_{i}$.
%	
%%	\begin{equation}
%%		D_{i}+\delta \geq d_{i},  \quad i \in \{1, 2\}.
%%	\end{equation}	
%%	Alternatively, we may occasionally say that the tuple $(b, D_{1}, D_{2})$ is achievable if the latency $b$ is $(D_{1}, D_{2})$-achievable.
%	
%%The achievable latency region is the set of all achievable latencies under the prescribed distortion vector.
%
%\end{mydef}

\begin{remark}
	In our work, we assume that the latency $b > 1$, since otherwise, finding matching inner and outer bounds are trivial~\cite{TLKS_TIT16} for the case when $b \in (0, 1]$.
\end{remark}

Finally, in our outer bound, we consider only the class of non-erasure-randomized codes, which assumes that the positions of non-erased symbols in the reconstruction of $\SHatK{2}$ given $\YW$ depends only on the channel noise realization $\NW$, and not on the actual channel output \YW.  
That is, we assume that the decoder for the weaker user, user~2, is such that given \NW, which specifies the positions of the erasures in the channel output, the positions of the reconstructed source symbols are determined.  We formally define this below.
%That is, we assume that given \nN{0} and the position of the erasures in the channel output, \nN{i} can be deterministically constructed and consequently, the positions of the reconstructed source symbols, as indicated by $R_i$ are deterministic so that $R_i = f(N_0^n)$.

\begin{mydef}
\label{def:non_erasure_randomized}
	Let $\YW$ be the channel output of user~2.  An $(m, n, d_1, d_2)$ code is said to be non-erasure-randomized if for every $\nN{0} \in \{0,1\}^n$, there exists a predetermined set $R(\nN{0}) \subseteq [m]$ such that the reconstruction 
%	$\tSM{0} = g_{i, m}(\YW)$ satisfies
	$\SHatK{2} = g_{i, m}(\YW)$ satisfies
	
	\begin{enumerate}
		\item $\SHatK{2}(k) = \star$ for all $k \in [m] \setminus R(\nN{0})$
		\item $\SHatK{2}(j) = S^m(j)$ for all $j \in R(\nN{0})$.
	\end{enumerate}
\end{mydef}

%\begin{remark}
%\label{rem:deps}
%Throughout this paper we will assume that for each user $i \in [n]$, we have that $d_i < \epsilon_i$. Any user $j$ with $d_j \ge \epsilon_j$ will be trivially satisfied by the systematic portion of our segmentation-based coding scheme.  Furthermore, we will show in Lemma~\ref{lem:bn1} that within our class of coding schemes, such a systematic portion can be transmitted without loss of optimality when at least one user satisfies $d_i < \epsilon_i$. Finally, if every user satisfies $d_i \ge \epsilon_i$, a simple uncoded transmission scheme is easily shown to be optimal.
%\end{remark}

%\begin{remark}
%	While our system model has assumed binary alphabets for both source and channel input sequences, our results can easily be extended to larger alphabet sizes.  {Provided we keep source and channel input alphabets identical in size, our results could then extend to packet erasure networks.}
%\end{remark}


%For convenience, throughout this paper, for any positive integer $k$, we shorthand the set $\{1,2,\dots,k\}$ as $[k].$
%
%Consider broadcasting a length-$N$ binary sequence $S = \{s(j)\}_{j\in[N]}$ from a source to $n$ receivers over independent memoryless binary erasure channels. For $i\in[n]$, denote the erasure rate of the channel between the source and receiver $i$ as $\epsilon_i$. Applying some encoding scheme to $S$, the source generates and broadcasts the coded binary sequence $X=\{x_j\}_{j\ge1}$. Each receiver $i$ retrieves from the channel a sequence $Y^i = \{y_{j}^i\}_{j\ge1}$ where $y_{j}^i \in \{0,1,e\}$, $e$ indicating an erasure. Denote $Y^{i,W} = \{y_{j}^i\}_{j\in[W]}$ as the truncation of $Y^i$ up to the $W$th symbol. Receiver $i$ reconstructs from $Y^{i,W}$ a copy $\hat S^{i,W}=\{\hat s_{j}^{i,W}\}_{j\in[N]},$ where $\hat s_{j}^{i,W}\in\{0,1,e\}.$
%
%%\subsection{Erasure Distortion}
%We consider a symbol-by-symbol based erasure reconstruction distortion measure $D_e: \{0,1\}\times \{0,1,e\}\mapsto \mathds R$ defined as
%\begin{align*}
%D_E(s,\hat s) = \left\{\begin{array}{lr} 0,& \textnormal{if } \hat s=s\\ 1, & \textnormal{if } \hat s\ne s, \hat s\ne e\\ \infty,& \textnormal{if } \hat s=e \end{array}\right.
%\end{align*}
%%for symbols $s\in\{0,1\}$ and $\hat s\in\{0,1,e\}$,
%and
%\begin{align*}
%D(S,\hat S^{i,W}) =  \frac{1}{N}\sum_{j\in[N]} D_E(s_j,\hat s_{j}^{i,W}).
%\end{align*}
%for the source sequence $S$ and the sequence $\hat S^{i,W}$ reconstructed by user $i$ from the first $W$ symbols of the channel output sequence $Y^{i,W}$.
%
%Now our problem is to upper bound and lower bound the minimum $W$, or $w=W/N,$ which we refer to as the {\it latency}, that guarantees $\mathds E[ D(S,\hat S^{i,W})]\le d_i$ for all $i\in[n]$,
%where $d_i$ is the given distortion requirement of user $i$.
%
%Clearly, $w$ is trivially lower bounded by $\max_{i\in[n]}\{\frac{1-d_i}{1-\epsilon_i}\}$. In the next section, we provide an upper bound of $w$ and the achieving coding scheme. We show that the upper bound is achieved with a coding scheme that sends a part of the source sequence uncoded, partitions the rest of the source sequence into a number of segments, and encodes each segment by a systematic optimal erasure code. The optimal segmentation can be found by solving a linear programming problem. We also show in Sec.~\ref{sec:jscc} that the segmentation-based scheme is equivalent to the Mittal-Phamdo~\cite{} scheme for erasure channels.

%\input{SysModel/individual_code}

%\input{SysModel/JSCC_approach3}









